A Catalog of the Most Optically Luminous Galaxies at z<0.3: Super Spirals, Super Lenticulars, Super Post-Mergers, and Giant Ellipticals

We present a catalog of the 1525 most optically luminous galaxies from the Sloan Digital Sky Survey (SDSS) with r-band luminosity L_r > 8L* and redshift z<0.3, including 84 super spirals, 15 super lenticulars, 14 super post-merger galaxies, and 1400 giant ellipticals. With mass in stars of 10^{11.3}-10^{12} M_sun, super spirals and lenticulars are the most massive disk galaxies currently known. The specific star formation rates of super spirals place them on or below the star-forming main sequence. They must have formed stars at a high rate throughout their history in order to grow their massive, gigantic stellar disks and maintain their blue u-r integrated colors. Their disks are red on the inside and blue on the outside, consistent with inside-out growth. They tend to have small bulge-to-total (B/T) r-band luminosity ratios, characteristic of disk building via minor mergers and cold accretion. A large percentage of super disk galaxies (41%) have double nuclei, double disks, or other signatures of ongoing mergers. Most (72%) are found in moderate to low density environments, while the rest are found at the outskirts of clusters. It is likely that super spirals survive in these environments because they continue to accrete cold gas and experience only minor mergers at late times, by virtue of their enormous masses and angular momenta. We suggest that super post-mergers are the product of super-spiral major mergers and may be the precursors of some giant elliptical galaxies found in low density environments. We present two new gravitational lens candidates in the Appendix.

==> ogle_paper_tableA1 <==
#-------------------------------------------------------------------------------
# J/ApJS/vol/page  A Catalog of the Most Optically Luminous Galaxies at z<0.3:
# Super Spirals,  Super Lenticulars,  Super Post-Mergers, and Giant Ellipticals
# (Ogle+2019)
#-------------------------------------------------------------------------------
#-- Table J/ApJS/vol/page/TableA1 The Ogle et al. Galaxy Catalog (OGC)
#-------------------------------------------------------------------------------
# Label     Format   Unit    Explanations
#-------------------------------------------------------------------------------
# OGC       I4       ----    Ogle et al. galaxy catalog identifier
# NED_Name  A33      ----    NASA Extragalactic Database preferred name
# L_r       F5.1     L*      SDSS r-band luminosity, k-corrected, and divided by L*=5.41 \times 10^{43}$ erg s$^{-1}$ at 6200 \AA
# r         F5.2     AB mag  SDSS r-band CModel magnitude
# z_NED     F8.6     ----    NED preferred redshift, primarily from SDSS DR6
# Morph.    A6       ----    Galaxy morphology: G  =  unclassified galaxy, E  =  elliptical, Epec  =  peculiar elliptical, dE  =  dwarf elliptical, S0  =  lenticular,  S  =  spiral, SS  =  super spiral, Pec  =  peculiar, GLens  =  gravitational lens.
#-------------------------------------------------------------------------------
#-------------------------------------------------------------------------------
OGC     NED_Name                         L_r      r       z_NED      Morph.
0021    2MASX J12220526+4518109           19.8    16.26   0.264357   E   
0022    B3 1715+425                       19.5    15.34   0.182900   E  
0023    SDSS J215541.97+123128.5          19.1    15.68   0.193000   E  
0028    2MASX J14550676+6158093           17.2    16.51   0.274216   E  
0029    2MASX J09501212+2138520           16.8    16.54   0.271226   E  
0032    MCG +04-28-097                    16.1    14.93   0.142912   E  
0033    2MASX J11561081-0021011           16.0    16.44   0.256380   E  
0034    2MASX J14010204+0252423           16.0    16.41   0.251982   E  
0037    2MASX J08265755+3108044           15.7    15.97   0.209455   E  
0039    2MASX J17120987+6143147           15.5    15.45   0.172870   E  
0040    2MASX J08252902+4707598           15.4    14.75   0.129069   E  
0041    2MASX J09093863+5133268           15.2    16.79   0.288775   E   
0042    2MASX J12432467+2716501           15.2    15.78   0.197000   E   
0043    2MASX J08425763+3622000           15.1    16.79   0.282265   E   
0044    2MASX J14072225+1352512           15.1    16.86   0.293596   SS  
0046    2MASX J10170363+3902500           14.9    15.91   0.205544   E   
0047    2MASX J09110566+6107477           14.9    16.78   0.279000   E   
0049    2MASX J17132838+2743362           14.8    16.95   0.297179   E   
0050    LCRS B143146.7-021941             14.8    16.93   0.290459   E   
0051    2MASX J11415986+2503026           14.8    16.70   0.274309   E   
0053    2MASX J11142408+1309217           14.6    16.83   0.287909   E      
0054    2MASX J12012247+2351103           14.6    16.32   0.236192   E      
0055    2MASX J22125523-0746477           14.5    16.16   0.215903   E      
0058    2MASX J14431968+2748461           14.4    16.63   0.264000   E     
0060    2MASX J02203298+0028032           14.2    16.76   0.272092   E     
0061    2MASX J15070153+1052566           14.1    17.00   0.296000   E     
0062    2MASX J11082297+2914281           14.1    16.08   0.212296   E     
0064    2MASX J15015744+2212596           14.0    16.69   0.260000   E     
0065    2MASX J10301576-0106068           13.9    16.92   0.282251   SS    
0066    2MASX J11321396+1118481           13.8    16.80   0.273074   E     
0067    2MASX J16241402+4114377           13.7    15.70   0.183253   E     
0068    2MASX J09562806+1831023           13.6    15.41   0.160811   E     
0070    2MASX J08005684+3603234           13.5    17.00   0.287310   E     
0071    2MASX J09122151+2129546           13.5    16.84   0.272859   E     
0072    2MASX J17304291+6227468           13.4    15.82   0.185876   E     
0073    2MASX J10405643-0103584           13.4    16.64   0.250303   SS    
0075    2MASX J00313409-1045488           13.4    16.71   0.262302   E     
0077    SDSS J085608.51+541854.8          13.3    16.66   0.259429   E    
0078    2MASX J02295551+0104361           13.3    16.53   0.245472   E     
0079    2MASX J10184324+1244103           13.3    15.99   0.195885   E    
0080    2MASX J15073793+3946094           13.2    16.55   0.250035   E    
0081    2MASX J14592775+0320461           13.2    16.87   0.271529   E    
0082    2MASX J13165534+2615299           13.2    16.95   0.289802   E    
0083    2MASX J12055905+1004483           13.1    16.41   0.233693   E    
0084    2MASX J12281614+4950223           13.0    16.71   0.263700   E    
0085    2MASX J11375950+5723031           13.0    16.97   0.290921   E    
0086    2MASX J17201001+2637317           13.0    15.52   0.160114   E    
0087    LCRS B150131.5-023636             13.0    16.42   0.217077   E     
0088    2MASX J13150513+5149022           12.9    16.92   0.283600   E    
0089    2MASX J08554018-0032569           12.9    16.84   0.270660   E    
0090    2MASX J12341746+0945577           12.9    16.39   0.230611   E    
0091    2MASX J10253527+5105541           12.9    15.14   0.141878   E    
0092    2MASX J12114313+0801071           12.8    16.57   0.248170   E    
0093    2MASX J12011702+4750038           12.8    16.83   0.272062   E    
0094    2MASX J13074925+2925484           12.8    16.48   0.240416   E    
0095    2MASX J10144944+1039234           12.8    16.02   0.197506   E    
0096    2MASX J10292509+3737478           12.8    15.27   0.149000   E    
0097    2MASX J11330294+3946524           12.8    17.03   0.292296   E    
0098    WISE J212939.98+000521.9          12.8    16.48   0.233962   E    
0099    MCG +10-19-068                    12.7    14.63   0.115410   E    
0100    SDSS J111157.67-003922.1          12.7    16.96   0.279864   E    
0101    2MASX J10232077+5948393           12.7    15.98   0.198899   E   
0103    2MASX J12001112+6809250           12.7    16.75   0.262837   E   
0104    2MASX J12460941+5150211           12.7    16.80   0.269660   E   
0105    2MASX J10181744+1209219           12.6    16.56   0.240673   E   
0106    2MASX J02235913-0835405           12.6    16.88   0.270577   E   
0107    2MASX J13543126+0401377           12.6    16.71   0.256618   E   
0108    2MASX J14535141+5723366           12.6    16.91   0.279715   E   
0109    2MASX J13560242+0210449           12.6    16.79   0.262699   E   
0110    4C +41.26                         12.6    16.35   0.227800   E   
0111    2MASX J08224123+1759129           12.5    17.13   0.296769   E   
0112    2MASX J14422796+3234438           12.5    16.52   0.240942   E   
0113    LCSB S1044O                       12.5    15.70   0.168041   E   
0114    2MASX J11423258+5056248           12.4    16.73   0.260317   E   
0115    2MASX J11051814+0653193           12.4    16.52   0.234418   E   
0116    2MASX J10052605+5058409           12.4    16.38   0.227643   E   
0117    SDSS J101017.34+324954.6          12.3    17.05   0.292039   E   
0118    2MASX J10535025+1651022           12.3    13.95   0.083784   E   
0119    SDSS J124822.79+284315.0          12.3    16.52   0.239590   E   
0120    2MASX J09594676+2224099           12.3    16.60   0.244674   E   
0121    2MASX J11071387+3315020           12.3    16.67   0.251328   E   
0122    2MASX J08373437+1549073           12.3    15.39   0.152610   E   
0123    PKS 2338+000                      12.3    16.94   0.276739   E    
0125    SDSS J104044.49+395711.2          12.3    15.14   0.138000   E   
0126    2MASX J14464688+1606440           12.3    16.22   0.211497   E   
0127    2MASX J08293387+0840013           12.3    16.75   0.258096   E   
0128    2MASX J13064997+4633335           12.2    16.45   0.233000   E   
0129    2MASX J10122067+5701171           12.2    17.05   0.290736   E   
0130    2MASX J13225878+0954454           12.1    16.43   0.228204   E   
0131    2MASX J14582478+4842369           12.1    16.13   0.204411   E   
0132    2MASX J13042885+6439373           12.1    16.52   0.235245   E   
0133    2MASX J13433788+4946263           12.1    16.86   0.270999   E   
0134    IC 2657                           12.1    15.65   0.167932   E   
0135    2MASX J09322275+0811508           12.1    16.05   0.192506   E   
0136    2MASX J15241951+3515592           12.0    16.70   0.252535   E   
0137    CGCG 078-079                      12.0    13.64   0.071770   E   
0138    2MASX J16161819+0700331           12.0    16.80   0.253693   E   
0139    2MASX J16394598+4609058           12.0    16.63   0.247342   SS  
0140    2MASX J09503021+5735027           12.0    17.00   0.284530   E   
0141    2MASX J10521000+1034056           12.0    16.35   0.220168   E   
0142    2MASX J08403267+0542464           12.0    16.98   0.273984   E   
0143    2MASX J11441130+0055210           12.0    17.16   0.298286   E   
0144    2MASX J13141970-0127257           12.0    15.85   0.180190   E   
0145    2MASX J16124326+4152441           11.9    17.14   0.298727   E   
0147    2MASX J15354520+0004590           11.9    17.26   0.295364   E    
0148    2MASX J09452329+4236037           11.9    17.02   0.284734   E    
0149    2MASX J11120065+3341192           11.9    16.68   0.248970   E    
0150    SDSS J152242.72+574009.4          11.9    16.11   0.202026   E    
0151    B2 0916+36A                       11.9    16.38   0.223743   E    
0152    2MASX J10413089+5424409           11.8    17.04   0.287599   E    
0153    2MASX J11185137+1113392           11.8    16.61   0.242517   E    
0154    2MASX J14304531+2025428           11.8    16.85   0.262000   E    
0155    2MASX J16193879+0946002           11.8    16.62   0.236703   E    
0156    2MASX J12053162+1526435           11.7    16.37   0.218902   E    
0157    2MASX J15292202+0927536           11.7    17.22   0.299637   E    
0158    2MASX J13341844-0057248           11.7    16.93   0.270378   E    
0159    2MASX J12280342+3759557           11.7    16.75   0.256569   E    
0160    2MASX J10224346+3218367           11.7    17.06   0.286223   E    
0161    2MASX J11384473+1028254           11.7    16.83   0.257660   E    
0163    2MASX J13280533+0917230           11.7    16.51   0.232131   E    
0164    2MASX J10160950+1158015           11.7    16.62   0.238462   E    
0165    2MASX J12364401+5254415           11.7    16.95   0.274696   E    
0166    SDSS J134030.19+411536.5          11.7    16.77   0.258606   E    
0167    2MASX J11452628+1112310           11.7    16.94   0.270333   E    
0168    2MASX J21113345-0550252           11.6    17.13   0.274724   E    
0169    2MASX J08255782+0414480           11.6    16.45   0.225130   E    
0170    2MASX J10100707+3253295           11.6    17.10   0.289913   SS   
0171    2MASX J15292880+1859110           11.6    16.38   0.211772   E    
0173    2MASX J09274787+2314060           11.5    16.79   0.255329   E    
0174    2MASX J09401837+2920057           11.5    16.92   0.269320   E    
0175    2MASX J14522366+6117075           11.5    16.98   0.278920   E    
0176    2MASX J09182135+6110290           11.5    17.05   0.279000   E    
0177    2MASX J00300134+1417258           11.5    16.36   0.207550   E    
0178    MCG +00-60-013                    11.5    14.07   0.084295   E    
0179    SDSS J213701.13-064447.0          11.5    17.16   0.290697   SS  
0180    2MASX J08123405+4937423           11.5    16.68   0.238437   E    
0181    2MASX J13270101+0212189           11.5    16.84   0.260141   E    
0182    2MASX J09323937+3753141           11.5    16.01   0.190975   E    
0183    2MASX J11245231+4140029           11.5    16.10   0.197276   E    
0184    2MASX J11540477+0036186           11.5    16.49   0.228773   E    
0185    2MASX J14255668+3748589           11.4    15.73   0.170002   E    
0186    2MASX J15065893+1559585           11.4    16.75   0.251000   E    
0187    2MASX J11014714+2828080           11.4    16.82   0.255757   E    
0188    2MASX J16143111+2643504           11.4    15.99   0.184287   E    
0189    2MASX J09091273+1058286           11.4    15.88   0.176287   E    
0190    2MASX J22072433-0846313           11.4    17.18   0.292948   E    
0192    2MASX J10110772+1604457           11.4    15.36   0.143466   E    
0193    2MASX J13105635+2157562           11.4    17.06   0.282000   E    
0194    2MASX J14512953+4235352           11.4    16.20   0.204397   E    
0195    2MASX J09194427+5622012           11.4    17.05   0.277908   E    
0196    2MASX J13524570+6012012           11.4    17.13   0.291714   E    
0197    2MASX J11232451+0712317           11.3    17.12   0.273990   E    
0198    2MASX J14471870+4248163           11.3    16.41   0.222023   E    
0199    2MASX J12081059+2426491           11.3    16.87   0.260000   E    
0200    2MASX J08355126+3926220           11.3    16.90   0.260347   E     
0201    2MASX J15342642-0119003           11.3    15.71   0.154323   E    
0202    SDSS J101619.36-013552.1          11.3    16.93   0.263500   E    
0203    2MASX J11125450+1326093           11.3    15.72   0.168483   E      
0204    2MASX J14480549+1841271           11.3    17.09   0.281000   E    
0205    2MASX J14162734+2315222           11.2    15.23   0.138000   E    
0206    SDSS J153344.13+033657.5          11.2    17.23   0.292844   E    
0207    2MASX J10233480+0336336           11.2    16.32   0.210154   E    
0208    SDSS J092216.08+122554.2          11.2    16.00   0.185689   E    
0209    2MASX J11341384+3955203           11.2    17.17   0.292677   E    
0210    2MASX J11414428+2653236           11.2    17.20   0.294819   E    
0211    2MASX J14371203+2044542           11.2    16.76   0.248794   E    
0212    2MASX J14410242+4336544           11.2    17.12   0.286629   E    
0213    2MASX J12020669-0014293           11.2    16.75   0.249028   E    
0214    2MASX J13114620+2201367           11.2    15.78   0.171501   E    
0215    2MASX J21475496-0737536           11.2    17.19   0.287071   E    
0216    2MASX J21454034-0805374           11.2    15.87   0.171155   E    
0217    2MASX J13275756+3345291           11.2    16.72   0.248949   SS   
0218    2MASX J09355768+2326063           11.2    16.82   0.254033   E    
0219    CGCG 168-022                      11.2    14.42   0.098278   E    
0220    2MASX J21302696-0000242           11.2    15.27   0.137518   E    
0221    2MASX J12553165+3520493           11.2    15.61   0.161000   E    
0222    2MASX J12220815+4844557           11.1    17.22   0.298603   SS    
0223    2MASX J01024765+1556578           11.1    17.18   0.280644   E    
0224    2MASX J15302921+2123011           11.1    16.81   0.245542   E    
0225    2MASX J16111703+3139131           11.1    17.07   0.278271   E    
0226    2MASX J11243877+0127158           11.1    16.62   0.233010   E    
0227    SDSS J163403.72+251734.8          11.1    17.00   0.269815   E       
0228    SDSS J093839.24+142708.2          11.1    15.95   0.177802   E    
0229    2MASX J17231311+5618082           11.1    16.60   0.234172   E    
0230    2MASX J10324283+2853551           11.1    17.20   0.293926   E    
0231    2MASX J16061376+2008062           11.1    15.90   0.173153   E    
0232    2MASX J11152967+2050433           11.1    16.21   0.202458   E    
0233    2MASX J10385227+2903198           11.1    17.00   0.272812   E    
0234    2MASX J14391300+5849206           11.1    16.63   0.241104   E    
0235    2MASX J14222262+6023160           11.0    16.52   0.229984   E    
0236    2MASX J12105875+3845153           11.0    16.94   0.265744   E    
0237    2MASX J13225446+5810030           11.0    16.09   0.194475   E    
0238    2MASX J08474073+2931278           11.0    16.21   0.198043   E    
0239    2MASX J11552373+1507564           11.0    17.19   0.287800   G       
0240    2MASX J11581174+0900258           11.0    17.18   0.292201   E    
0241    2MASX J15351941+3421287           11.0    16.61   0.234733   E    
0242    2MASX J12293088+1544029           11.0    16.77   0.247674   E    
0243    2MASX J11400562+1813240           11.0    15.01   0.124359   E    
0244    2MASX J13365650+3326044           10.9    16.71   0.245337   E    
0245    2MASX J12285430+1925548           10.9    15.66   0.160961   E    
0246    2MASX J14403874+3727267           10.9    16.86   0.260421   E     
0247    SDSS J081953.52+041409.2          10.9    17.24   0.296625   Epec  
0248    2MASX J12141371+2637584           10.9    15.72   0.165474   E   
0250    2MASX J14283842+5651381           10.9    14.60   0.105967   E   
0251    2MASX J13064625+3947510           10.9    14.69   0.109497   E   
0252    2MASX J09055769+4057394           10.9    16.67   0.240821   E   
0253    ABELL 1882 BCG                    10.9    15.33   0.138983   E   
0255    2MASX J10320551+3352007           10.9    17.02   0.273999   E   
0256    2MASX J11593546+1257080           10.9    16.95   0.263572   SS  
0258    2MASX J07524164+3356595           10.8    17.13   0.277212   E   
0259    2MASX J12415037+1946558           10.8    17.16   0.287000   E   
0260    2MASX J09474943+1148374           10.8    17.27   0.298817   E   
0261    2MASX J10532815+3708507           10.8    17.05   0.277438   E   
0262    2MASX J15331120+3820054           10.8    17.05   0.277390   E   
0263    2MASX J13170725+6039010           10.8    16.72   0.245000   E   
0264    B2 1003+26                        10.8    14.90   0.116838   E   
0265    SDSS J115052.98+460448.1          10.8    17.18   0.289538   SS  
0266    2MASX J11440384+4400214           10.8    17.28   0.299157   E   
0267    2MASX J09175344+5143379           10.8    16.41   0.217253   E   
0268    2MASX J10370788+6014523           10.8    16.52   0.227551   E   
0269    2MASX J11560809+4410580           10.8    17.24   0.297048   E   
0271    2MASX J13105976+6354110           10.7    15.18   0.132709   E   
0272    2MASX J12352690+6320328           10.7    16.88   0.260344   E   
0274    2MASX J14072147-0010266           10.7    16.95   0.261314   E    
0275    2MASX J15154814+5655072           10.7    17.21   0.293191   E    
0276    2MASX J10581332+2808071           10.7    16.40   0.214616   E    
0277    2MASX J15463914+0124226           10.7    16.50   0.208379   E    
0278    2MASX J16354844+1503073           10.7    17.32   0.291875   E    
0279    2MASX J23183035+0105318           10.7    17.02   0.262882   E    
0280    2MASX J09572689+4918571           10.7    16.68   0.241492   SS    
0281    2MASX J23034643+1523006           10.7    16.95   0.245966   E    
0282    2MASX J14490790+1448598           10.7    16.51   0.223885   E    
0283    2MASX J12043513+0357226           10.7    15.70   0.162636   E    
0284    SDSS J212436.75-003119.7          10.7    16.69   0.234995   E    
0285    2MASX J14485785+5839379           10.7    17.25   0.297862   E    
0286    2MASX J10222849+5006200           10.7    15.60   0.158000   E    
0287    2MASX J03311855-0604297           10.7    16.99   0.261547   E    
0288    2MASX J14015177+0222149           10.6    16.85   0.251798   E    
0289    2MASX J10074257+3800462           10.6    14.77   0.112051   E    
0290    2MASX J12343099+5156295           10.6    17.25   0.295982   SS    
0291    2MASX J11113716+0413104           10.6    16.84   0.247552   E    
0292    SBS 1638+538                      10.6    14.75   0.110046   E    
0293    2MASX J13044128+6635345           10.6    17.18   0.288630   SS    
0294    2MASX J01431651+0058235           10.6    15.80   0.167074   E    
0295    2MASX J15482746-0058341           10.6    16.81   0.230533   E    
0296    2MASX J15423606+5428545           10.6    17.10   0.280747   E    
0297    2MASX J14533803+2650234           10.6    17.12   0.277000   E    
0298    2MASX J14332826+0606013           10.6    16.73   0.239016   E    
0299    2MASX J09094480+2226078           10.5    17.25   0.285386   SS  
0300    B3 1424+423                       10.5    15.14   0.130000   E    
0301    2MASX J08362624+0643355           10.5    17.04   0.268713   E    
0302    2MASX J15430777+1937522           10.5    16.67   0.228909   G    
0303    2MASX J16320739+2146018           10.5    16.10   0.185675   E    
0304    SDSS J105417.54+143904.1          10.5    17.31   0.299475   E      
0305    2MASX J14381668+4035303           10.5    16.42   0.215906   E    
0306    SDSS J122100.48+482729.1          10.5    17.29   0.299787   SS    
0307    SDSS J143335.34+242039.2          10.5    17.27   0.292796   Ex2      
0308    2MASX J08243684+2242034           10.5    17.18   0.280168   E    
0309    2MASX J02591402-0037150           10.5    16.39   0.194282   E    
0310    2MASX J13405808+5802419           10.5    15.17   0.132158   E    
0311    2MASX J09443173+2815579           10.4    17.08   0.274931   E    
0312    2MASX J09350306+2435466           10.4    16.91   0.258305   E    
0313    2MASX J09013009+5539166           10.4    14.87   0.115525   E    
0314    2MASX J12021953+1125493           10.4    16.28   0.202123   E    
0315    2MASX J13581072+3301321           10.4    17.17   0.286000   E    
0316    2MASX J16024324+3250384           10.4    17.24   0.288079   E    
0317    2MASX J15233340+4503354           10.4    16.87   0.253052   E    
0318    2MASX J12055981+6208348           10.4    17.04   0.270751   E    
0319    2MASX J10074437+2007479           10.4    16.85   0.250125   E    
0320    2MASX J14440908+0010428           10.4    17.35   0.296640   E    
0321    2MASX J13045236+3533190           10.4    15.71   0.163279   E    
0322    2MASX J12535781+1933138           10.4    17.01   0.268000   E    
0323    2MASX J08250387+2355201           10.4    17.08   0.269413   E    
0324    2MASX J14331019+2030326           10.4    16.86   0.249279   E    
0325    2MASX J09133415+5001508           10.4    16.01   0.183270   E    
0326    2MASX J11250803+0259316           10.4    16.99   0.261657   E    
0327    2MASX J07365908+1716228           10.4    16.26   0.199000   E    
0328    2MASX J15250551+3326518           10.4    15.06   0.124278   E    
0329    2MASX J11421323+1154218           10.4    15.61   0.152541   E    
0330    2MASX J09204829+3028179           10.4    17.22   0.288270   E    
0331    SDSS J091318.25+492556.3          10.4    17.28   0.296414   Epec   
0332    2MASX J11331462+6622454           10.4    14.84   0.114799   E    
0333    2MASX J01020558+1542095           10.3    17.33   0.279735   E    
0334    2MASX J02063507+1330583           10.3    16.47   0.207659   E    
0335    2MASX J11105301+0714018           10.3    16.54   0.220576   E    
0336    2MASX J12584149-0145410           10.3    14.13   0.084565   E    
0337    PKS 2229-08                       10.3    14.18   0.083138   E    
0338    2MASX J13261515+2757490           10.3    16.87   0.254784   E    
0339    2MASX J10040332+3342321           10.3    16.23   0.199471   E    
0340    SDSS J100550.69+105811.6          10.3    15.77   0.161995   E    
0341    2MASX J14294016+2701274           10.3    17.00   0.266933   E    
0342    2MASX J13114905+3232306           10.3    16.80   0.248565   E    
0343    2MASX J12593908+2906207           10.3    15.74   0.165100   E    
0344    2MASX J01532569-0109358           10.3    16.77   0.241722   E     
0345    2MASX J09260805+2405242           10.3    16.57   0.222451   SS    
0346    2MASX J21522128-0719458           10.3    16.04   0.181155   E    
0347    2MASX J15150411-0047237           10.3    15.11   0.120731   E    
0348    2MASX J10261107+3239242           10.3    16.73   0.239800   E    
0349    2MASX J13322121+4102064           10.3    15.80   0.169125   E    
0350    SDSS J121711.23+344952.3          10.3    17.12   0.279542   E    
0351    2MASX J15450141+3231534           10.3    16.48   0.216703   E    
0352    2MASX J09185025+0212033           10.3    17.20   0.284003   E    
0353    2MASX J12230565-0152303           10.3    17.20   0.284020   E    
0354    2MASX J12461633+5004101           10.2    16.64   0.231983   E    
0355    2MASX J14370040+1154534           10.2    15.72   0.160694   E    
0356    2MASX J12115109+4849111           10.2    17.29   0.294216   E    
0357    2MASX J12285018+3823150           10.2    16.90   0.257051   E    
0358    2MASX J08480536+3044373           10.2    17.29   0.290239   E    
0359    2MASX J12271170+0352008           10.2    16.74   0.240074   E    
0360    2MASX J23031676-0051142           10.2    17.11   0.269000   E    
0361    2MASX J17041819+6159243           10.2    15.61   0.153688   E    
0362    2MASX J13204804-0026377           10.2    16.50   0.218947   E    
0363    2MASX J10544765+0907190           10.2    15.86   0.167951   E    
0364    SDSS J140912.42+311005.0          10.2    16.07   0.186500   E    
0365    2MASX J01220259+0020041           10.2    15.95   0.174497   E    
0366    2MASX J15090010+0023272           10.2    16.90   0.246995   E    
0367    2MASX J10395117+3826180           10.2    17.33   0.298662   E    
0368    2MASX J07513529+2610182           10.2    17.29   0.291440   E    
0369    2MASX J14183702+1446357           10.2    16.50   0.219015   E    
0370    2MASX J09340847+6145442           10.2    16.68   0.230582   E    
0371    2MASX J10215017+1407200           10.2    16.86   0.246007   E    
0372    2MASX J16433999+3019356           10.2    15.38   0.139343   E      
0373    2MASX J08195456+5634354           10.2    17.23   0.272878   E    
0374    2MASX J15570785+2024163           10.2    16.83   0.243200   E    
0375    2MASX J14443179+3113354           10.2    16.66   0.233300   E    
0376    2MASX J08425596+2927272           10.2    16.35   0.198003   E    
0377    2MASSi J2342593+134750            10.2    17.43   0.299123   G 
0378    2MASX J22165431-0947158           10.2    17.44   0.299206   E 
0381    2MASX J15521380+2013436           10.2    15.38   0.135660   E    
0382    2MASX J07255712+4123069           10.2    14.94   0.111314   E    
0383    2MASX J16231344+5000468           10.1    17.25   0.288973   E    
0384    2MASX J12183396-0210367           10.1    17.33   0.295709   E    
0385    2MASX J12560211+6624362           10.1    16.71   0.236365   E    
0386    2MASX J13572664+5709152           10.1    16.43   0.214167   E    
0387    2MASX J13562270+0339078           10.1    17.01   0.261828   E    
0388    2MASX J17340613+6029190           10.1    17.19   0.275807   SS  
0389    2MASX J09561919+2811573           10.1    16.27   0.199593   E    
0390    2MASX J14455826+4901050           10.1    17.28   0.290184   E    
0391    2MASX J17135225+5815516           10.1    16.80   0.241143   E    
0392    2MASX J13412540-0102300           10.1    17.25   0.286378   E    
0394    2MASX J16303925+3143314           10.1    16.43   0.211544   E    
0395    2MASX J13362703+5453538           10.1    14.70   0.106811   E    
0396    2MASX J14495360+3534570           10.1    17.28   0.293534   E    
0397    2MASX J11573825+2044409           10.1    15.46   0.144166   E    
0398    2MASX J11382476+1440305           10.1    16.61   0.223105   E    
0399    2MASX J08291232+3319054           10.1    16.90   0.249226   E    
0400    2MASX J02483875+0044261           10.1    16.81   0.238429   E    
0401    2MASX J13374081+4059547           10.1    17.23   0.289410   E    
0402    2MASX J11012817+0555019           10.1    17.02   0.263574   E    
0403    MCG +04-23-001                    10.1    16.23   0.191991   E    
0404    2MASX J14371672+1616048           10.1    17.04   0.266000   E    
0405    2MASX J09204322+0953162           10.1    16.93   0.249663   E    
0406    2MASX J16403246+4629049           10.1    16.65   0.230006   E    
0407    SDSS J082504.57+315957.1          10.1    17.08   0.264900   E    
0408    2MASX J21101927+0950467           10.1    16.81   0.230731   E    
0409    2MASX J13450104+4047508           10.0    16.91   0.256483   E    
0410    2MASX J13310330+5051045           10.0    16.23   0.197480   E    
0411    2MASX J09211110+3451352           10.0    16.73   0.237569   E    
0412    2MASX J14320098+2932534           10.0    16.51   0.218914   E    
0413    2MASX J14282026+3949489           10.0    15.78   0.165738   E    
0414    2MASX J09173962+5436415           10.0    16.54   0.220312   E      
0415    2MASX J11171016+2524099           10.0    16.89   0.253015   E    
0416    2MASX J14492864-0116172           10.0    16.40   0.202427   E    
0417    2MASX J11223616+5927053           10.0    16.91   0.256719   E    
0418    2MASX J12052321+1022461           10.0    14.45   0.095016   E    
0419    2MASX J12294828+2921012           10.0    17.16   0.278020   E    
0420    2MASX J12025420+1432552           10.0    16.93   0.252747   E    
0421    2MASX J13443180+3748505           10.0    16.07   0.185432   E    
0422    SDSS J130645.69+463330.7          10.0    16.50   0.218392   E    
0423    2MASX J10011749+1950090           10.0    17.35   0.297337   E    
0424    2MASX J14071738+1558082           10.0    15.20   0.129245   E    
0425    2MASX J21160443-0702228           10.0    16.40   0.191181   SS    
0426    2MASX J08593235+0308411           10.0    16.30   0.195981   E    
0427    2MASX J11594770+6752290           10.0    17.07   0.270384   E    
0428    2MASX J21173295+1004587           10.0    16.67   0.225510   E    
0429    2MASX J15415259+5042471           10.0    17.28   0.291856   E    
0430    2MASX J09113027+2945339           10.0    16.84   0.246128   E    
0431    B3 0920+408                       10.0    15.71   0.160196   E    
0432    2MASX J09414656+3919570           10.0    17.26   0.289073   E    
0433    2MASX J08152658+3959357           10.0    15.23   0.129000   E    
0434    2MASX J02375882-0109110            9.9    16.92   0.251211   E     
0435    2MASX J12553700+3456454            9.9    16.05   0.183038   E    
0436    2MASX J10111737+5934491            9.9    17.05   0.269704   E    
0437    2MASX J13130298+3519428            9.9    17.34   0.299163   E    
0438    2MASX J16462320+2018039            9.9    17.21   0.273578   E    
0439    2MASX J13443777+3810077            9.9    16.46   0.214481   E    
0440    2MASX J16095193+0714032            9.9    16.45   0.207071   E    
0441    SDSS J095727.02+083501.7           9.9    16.99   0.256568   SS    
0443    2MFGC 06756                        9.9    16.84   0.241071   E    
0444    VPC 0793                           9.9    15.92   0.171153   E    
0445    SDSS J101510.48+323150.7           9.9    17.25   0.288180   E    
0446    2MASX J16072379+3442099            9.9    17.25   0.286271   E    
0447    2MASX J08501347+6426231            9.9    15.50   0.138447   E    
0448    2MASX J12533274+6605143            9.9    16.72   0.234529   E    
0449    2MASX J09455221+5056386            9.9    16.86   0.248858   E    
0450    2MASX J20371439-0537504            9.9    17.02   0.256068   E      
0451    2MASX J14430657+0224069            9.9    15.43   0.138945   E    
0452    2MASX J15160704+1306184            9.9    16.76   0.233626   E    
0453    SDSS J120237.44+242903.4           9.9    16.53   0.218505   E    
0454    2MASXi J1003568+382901             9.9    16.97   0.258658   SS    
0456    2MASX J14331632+2200306            9.9    16.79   0.235682   E    
0457    2MASX J12195690-0051019            9.9    16.41   0.206557   E    
0458    2MASX J13012181+2402046            9.9    17.15   0.276000   E    
0459    2MASX J00281984+1354596            9.9    15.59   0.140821   E    
0460    2MASX J10224260+3325437            9.9    16.34   0.202375   E    
0461    2MASX J12470307+1833119            9.9    16.70   0.233598   E    
0462    2MASX J12184751+1204565            9.9    16.95   0.253889   E    
0463    2MASX J16280230+4635520            9.9    16.50   0.217143   E    
0464    2MASX J13025298+0332316            9.9    16.11   0.183871   E    
0465    2MASX J09230150+3326419            9.9    16.71   0.234538   E    
0466    2MASX J13133677+1745284            9.9    16.68   0.231236   E    
0467    2MASX J10253878+0407369            9.9    16.45   0.209668   E    
0468    2MASX J11463992+4851599            9.9    17.20   0.281665   E    
0469    SDSS J150022.77+220027.3           9.9    16.55   0.214069   Ex2       
0470    2MASX J13562044+1047238            9.9    16.80   0.240927   E    
0471    2MASX J14283237+1342062            9.9    15.72   0.158716   E    
0472    2MASX J12354758-0057575            9.9    15.49   0.144588   E    
0473    2MASX J13574191+4906328            9.8    16.62   0.226903   E    
0474    2MASX J13011647+2437472            9.8    16.70   0.234085   E    
0475    SDSS J143150.08+133204.9           9.8    15.75   0.159900   E    
0476    2MASX J12251073+1659109            9.8    16.69   0.230632   E    
0477    2MASX J15174560+2956299            9.8    17.28   0.288964   E    
0478    2MASX J12491863+5004489            9.8    16.87   0.249313   E    
0479    SDSS J093815.91+002109.1           9.8    17.30   0.281044   E    
0481    2MASX J16011418+4924421            9.8    16.86   0.246370   E    
0483    2MASX J13364941+1026239            9.8    15.70   0.155201   E    
0484    2MASX J12114773+2931222            9.8    17.10   0.270493   E    
0485    2MASX J12175677+2040163            9.8    16.33   0.200755   E    
0486    B3 1513+421                        9.8    15.35   0.134830   E    
0487    2MASX J00355515+0021236            9.8    17.00   0.259251   E    
0488    2MASX J13052154+1050013            9.8    17.14   0.273597   E    
0489    2MASX J14522021+2029154            9.8    17.20   0.277000   E    
0490    2MASX J12531675+2846231            9.8    16.17   0.190971   E    
0491    2MASX J13585168+3354341            9.8    17.21   0.282510   E    
0492    2MASX J08530543+2100349            9.8    16.73   0.232434   E    
0493    2MASX J14014604+0403139            9.8    16.95   0.253250   E    
0495    IC 1103                            9.8    14.12   0.079875   E    
0496    2MASX J15483160+1121489            9.8    16.71   0.225770   E    
0497    SDSS J113156.57+390628.2           9.8    16.72   0.231920   E    
0498    2MASX J14292941+0527494            9.8    17.20   0.278038   E    
0499    2MASX J15243000+3132092            9.8    16.46   0.210713   E    
0500    4C +54.16                          9.8    15.05   0.117520   E    
0501    2MASX J14384706+4419522            9.8    16.89   0.249354   E    
0502    2MASX J11092327+1524483            9.7    17.21   0.282261   E    
0504    SDSS J211356.48+104727.4           9.7    17.40   0.288075   E 
0505    2MASX J23160071-0951558            9.7    17.15   0.271565   E 
0506    2MASX J13044227+4002416            9.7    17.04   0.262287   E 
0507    2MASX J14480598+0521125            9.7    17.25   0.280419   E 
0508    2MASX J08592348+4927304            9.7    16.09   0.183075   E 
0509    2MASX J15012878+0336304            9.7    16.19   0.184618   E 
0510    2MASX J09122276+3106577            9.7    17.26   0.285941   E 
0511    2MASX J07591632+2812039            9.7    16.94   0.249067   E 
0512    2MASX J09121725+1935086            9.7    16.96   0.251399   E
0513    2MASX J15285081+1101439            9.7    16.67   0.225109   E   
0514    2MASX J10274899+4153140            9.7    15.94   0.174293   E   
0515    2MASX J12233272+6146195            9.7    16.97   0.256980   E   
0516    2MASX J14475296+1447030            9.7    16.57   0.220592   SS  
0517    2MASX J16265900+5528298            9.7    15.21   0.130000   E   
0518    2MASX J15020891+3331135            9.7    17.21   0.282054   E   
0519    2MASX J17190051+2909511            9.7    16.38   0.199106   E   
0520    SDSS J145400.58+103830.3           9.7    17.31   0.288778   E   
0521    2MASX J12154383+1709178            9.7    14.53   0.095633   E   
0522    2MASX J13511409+0147504            9.7    17.34   0.290536   E   
0523    2MASX J00515325+1504382            9.7    16.85   0.236371   E   
0524    2MASX J11422071+0547326            9.7    17.11   0.267178   E   
0525    2MASX J15582179+3151166            9.7    17.20   0.277914   E   
0526    2MASX J23233141-1025519            9.7    17.35   0.292096   E    
0527    2MASX J08322739+2838140            9.7    17.16   0.270823   E   
0528    2MASXi J0918567+341508             9.7    17.11   0.271111   E 
0529    2MASX J11464757+0952278            9.7    16.62   0.221403   E 
0530    2MASX J11204274+2231359            9.7    16.26   0.195091   E 
0531    2MASX J11041016+3016039            9.7    16.95   0.254413   E 
0532    2MASX J16415596+2113086            9.7    17.12   0.262632   E 
0533    B2 1113+24                         9.7    14.65   0.102100   E 
0534    2MASX J13311724+0727276            9.7    15.39   0.137097   E 
0535    SDSS J034217.22+000927.4           9.7    17.53   0.298391   E 
0536    LCSB S1936O                        9.6    16.04   0.176459   E
0537    2MASX J14420062+2523103            9.6    16.61   0.221099   E 
0538    B3 0911+418                        9.6    15.44   0.140639   E
0539    SDSS J093631.84+234235.4           9.6    16.47   0.209734   E 
0540    2MASX J09202502+0507097            9.6    17.16   0.265192   E 
0541    2MASX J02103254-0101252            9.6    17.30   0.285390   E 
0542    2MASX J15471905+3459399            9.6    16.26   0.193159   E 
0543    2MASX J09470010+2540462            9.6    14.83   0.109110   SS
0544    2MASX J13345435+4056552            9.6    16.76   0.238133   E 
0545    2MASX J14191718+4236543            9.6    16.89   0.249443   E 
0546    2MASX J11422228+2238500            9.6    16.08   0.179913   E 
0547    2MASX J14441440+3115273            9.6    16.74   0.235088   E 
0548    MCG +05-34-067                     9.6    15.26   0.131340   E 
0549    2MASX J15115064+1451041            9.6    16.17   0.185829   E 
0550    2MASX J08300363+0436360            9.6    16.53   0.214295   E 
0551    2MASX J09072119+2315556            9.6    16.86   0.240457   E 
0552    SDSS J121307.52+341034.2           9.6    16.66   0.227931   E    
0553    2MASX J09384773+5337591            9.6    16.36   0.202777   E    
0554    2MASX J10013116+2926334            9.6    16.90   0.249065   E    
0555    2MASX J23273191+0056346            9.6    17.25   0.278811   E    
0556    2MASX J08301911+2224044            9.6    17.45   0.298417   E    
0557    2MASX J11100726+4301468            9.6    15.70   0.156438   E    
0558    2MASX J14493336+3821424            9.6    15.44   0.141611   E    
0559    SDSS J095418.27+283011.0           9.6    16.38   0.202883   E    
0560    2MASX J08111642+2846529            9.6    17.16   0.270593   E    
0561    2MASX J13272292+0337454            9.6    16.65   0.224729   E    
0562    2MASX J02152418+1356196            9.6    17.54   0.292135   E    
0563    2MASX J09061369+1942538            9.6    16.73   0.229394   E    
0564    2MASX J10350012+3041380            9.5    15.39   0.137403   E    
0565    2MASX J02054883-0821285            9.5    16.86   0.243708   E    
0566    2MASX J09444319+0247541            9.5    16.66   0.220582   E    
0567    2MASX J13145492+5320363            9.5    17.20   0.276327   E    
0568    2MASX J08265518+4639174            9.5    17.41   0.295413   E    
0569    2MASX J12040355+2807050            9.5    15.88   0.166787   E    
0570    2MASX J08190976+2257125            9.5    16.63   0.219563   E    
0571    2MASX J12030545+5827444            9.5    17.19   0.276572   E    
0572    2MASX J15515285+0531592            9.5    17.02   0.250467   E    
0573    2MASX J13465566+1227510            9.5    17.00   0.255394   E    
0574    SDSS J121148.70+662514.4           9.5    16.79   0.237753   SS    
0575    2MASX J11222091+1211413            9.5    16.85   0.240906   E    
0576    2MASX J13374008+3858047            9.5    16.82   0.243606   E    
0577    2MASX J11583409+6422037            9.5    17.30   0.287368   E    
0578    MCG +00-60-005                     9.5    14.51   0.093521   E    
0579    2MASX J14371655+0945317            9.5    16.28   0.192116   E    
0580    SDSS J103739.06+100521.6           9.5    17.33   0.289000   E    
0581    2MASX J13423113+0021440            9.5    16.88   0.243520   SS+S      
0582    LCSB S1161P                        9.5    16.69   0.224486   E    
0583    SDSS J131842.65-024832.1           9.5    17.35   0.289949   E    
0584    2MASX J14335499+1016234            9.5    16.82   0.238764   E    
0585    CGCG 092-007                       9.5    16.02   0.174000   E    
0586    2MASX J11535621+4923562            9.5    15.90   0.166892   SS    
0587    2MASX J15081634+0019449            9.5    17.14   0.262775   E    
0588    2MASX J12344257+5857531            9.5    17.37   0.295524   E    
0589    2MASX J13405436+1108234            9.5    17.41   0.296955   E    
0590    2MASX J09372385+1253119            9.5    16.11   0.180128   E    
0591    2MASX J09411798+3311246            9.5    17.32   0.290252   E    
0592    2MASX J16040044+2813276            9.5    17.27   0.280455   E    
0593    2MASX J16523322+2842587            9.5    17.30   0.279616   E    
0594    LCRS B113856.0-022542              9.5    17.06   0.262546   E    
0595    2MASX J07550424+1353261            9.5    16.67   0.222669   SS    
0596    2MASX J12582791+6521303            9.5    16.75   0.234077   E    
0597    2MASX J11543710+1324046            9.5    17.33   0.287882   E    
0598    2MASX J09134494+4551329            9.4    16.14   0.186122   E    
0599    SDSS J131141.66+335917.9           9.4    16.87   0.246071   E    
0600    2MASX J03534263-0708280            9.4    16.47   0.196327   E    
0601    2MASX J16263208+4827461            9.4    16.23   0.191554   E    
0602    2MASX J21391954-0702320            9.4    16.51   0.207428   E    
0603    2MASX J15021906+1937381            9.4    17.28   0.279000   E    
0604    2MASX J11260451+5004109            9.4    17.32   0.289862   E    
0605    2MASX J09122599+0638237            9.4    16.83   0.234872   E    
0606    2MASX J13094818+1305435            9.4    16.09   0.179814   E    
0607    2MASX J10471907+2814348            9.4    16.91   0.246674   E    
0608    2MASX J09295240+0339592            9.4    16.93   0.245159   E    
0609    CGCG 064-024                       9.4    14.07   0.077707   E    
0611    2MASX J13163129-0105127            9.4    17.21   0.274343   E    
0612    SDSS J093540.34+565323.8           9.4    17.40   0.296393   SS    
0613    2MASX J14054313+1358118            9.4    17.41   0.297809   E    
0614    2MASX J11242304+1253164            9.4    17.29   0.282633   E    
0615    2MASXi J0837247+145819             9.4    17.26   0.278038   E      
0616    2MASX J11274328+4102052            9.4    16.34   0.199594   E    
0617    2MASX J14534324+2044364            9.4    15.03   0.115482   E    
0618    2MASX J15101172+3329112            9.4    14.89   0.111560   E    
0619    2MASX J10013337+3722377            9.4    17.16   0.273223   E    
0620    2MASX J09403051+6427236            9.4    16.87   0.236868   E    
0621    2MASX J14105487+2955291            9.4    16.02   0.176000   E    
0622    2MASX J14583507+3759333            9.4    16.34   0.199361   E    
0623    2MASX J09011007+2454570            9.4    17.00   0.252388   SS    
0624    2MASX J13245634+6219585            9.4    16.82   0.237397   Epec       
0625    2MASX J12070947+0424449            9.4    16.78   0.235321   E    
0626    2MASX J16264788+3610058            9.4    16.90   0.246714   E    
0627    2MASX J13241962+0419068            9.4    17.09   0.263073   E    
0628    4C +21.44E                         9.4    17.10   0.258000   E    
0629    2MASX J12084123+2941040            9.4    15.52   0.143833   E    
0630    2MASX J09421480+1522509            9.4    15.89   0.164176   E    
0631    2MASX J11355287+5103377            9.4    17.32   0.289253   E    
0632    2MASX J00295172+1402418            9.4    16.61   0.208934   E    
0633    2MASX J09470758+0044167            9.4    17.36   0.261902   E    
0634    NGC 5285                           9.4    13.88   0.072250   E    
0635    SDSS J143821.36+005308.0           9.4    17.29   0.279918   E    
0637    2MASX J15575566+4322473            9.3    16.43   0.206452   SS    
0638    2MASX J14502217+1857403            9.3    17.31   0.280000   E    
0639    2MASX J14595550+2307371            9.3    16.18   0.181230   E    
0640    2MASX J01334138+1339488            9.3    16.39   0.197114   E    
0641    2MASX J15583444+0759463            9.3    16.73   0.227840   E    
0642    2MASX J14060404+4041387            9.3    16.48   0.210987   E    
0643    2MASX J13454536+2827158            9.3    17.33   0.289162   E    
0644    2MASX J13182355-0031462            9.3    14.93   0.111829   E    
0645    2MASX J12474873+1038529            9.3    16.92   0.245715   E    
0646    2MASX J21193928+1039326            9.3    16.89   0.236746   E      
0647    2MASX J13225759+0701454            9.3    17.28   0.280448   E    
0648    2MASX J14150742+1710560            9.3    16.80   0.235920   E    
0649    2MASX J15445685+1705020            9.3    17.25   0.276000   E    
0650    LCRS B115038.8-024742              9.3    17.26   0.281257   E    
0651    2MASX J11241311+5133494            9.3    16.77   0.235108   E    
0652    2MASX J13040443+2052354            9.3    17.28   0.280000   E    
0653    2MASX J12181118+6240504            9.3    16.98   0.253247   E    
0655    2MASX J15470625+3307208            9.3    15.25   0.126704   E    
0656    SDSS J160712.03+354706.0           9.3    16.85   0.239668   E    
0657    2MASX J11353997+3009174            9.3    16.50   0.209948   E    
0658    2MASX J09151349+0502513            9.3    15.60   0.143556   E    
0659    2MASX J13443677+2446566            9.3    15.42   0.138196   E    
0660    SDSS J095551.61+110233.4           9.3    17.28   0.280970   E    
0661    2MASX J08491128+4735039            9.3    16.17   0.184776   E    
0662    2MASX J12024335+0358353            9.3    15.39   0.135497   E    
0663    UGC 08769                          9.3    13.70   0.066052   E    
0664    2MASX J09535418+2218509            9.3    17.12   0.264748   E    
0665    SDSS J105018.51+071855.6           9.3    17.46   0.299744   E    
0666    2MASX J00535416-0928230            9.3    17.20   0.270089   E    
0667    2MASX J10112972+0821053            9.3    17.21   0.274005   E    
0668    2MASX J17092557+5727012            9.3    15.24   0.126931   E    
0669    2MASX J13171572+3620513            9.3    16.89   0.245843   E    
0670    2MASX J11350037+0938000            9.3    17.47   0.299177   E    
0671    B2 1132+32                         9.3    16.75   0.230998   E    
0672    2MASX J13211578+2810411            9.3    17.23   0.279039   E    
0673    2MASX J12415739+0915419            9.3    16.70   0.227122   E     
0674    2MASX J12024238-0123455            9.3    16.94   0.248090   E    
0675    2MASX J02103987-0038312            9.3    17.35   0.287115   E    
0676    2MASX J14352846+5507519            9.3    15.46   0.140200   E    
0677    2MASX J11351879+1253111            9.3    16.45   0.204043   E    
0678    SDSS J230348.78-004023.9           9.3    17.19   0.266166   E    
0679    2MASX J08302686+3402239            9.3    17.08   0.258219   E    
0680    2MASX J00012634-0001437            9.3    16.96   0.248038   E    
0681    SDSS J092304.76+003119.9           9.3    17.46   0.299252   E    
0682    SDSS J161653.17+092635.6           9.3    16.47   0.202741   E    
0684    2MASX J08545745+3524513            9.3    15.55   0.143011   E    
0685    2MASX J11012592+5737199            9.3    16.81   0.239138   E    
0686    2MASX J13550747+3354588            9.3    17.27   0.281026   E    
0687    2MASX J10501260+3329225            9.3    17.18   0.272190   E    
0688    B3 1448+445                        9.3    17.32   0.286252   E    
0689    2MASX J15231620+0414569            9.3    15.74   0.152385   E    
0690    2MASX J12492211+4947419            9.3    17.31   0.286313   E    
0691    SDSS J121741.89+643510.3           9.3    15.37   0.133986   E    
0692    2MASX J12070909+0828467            9.3    16.73   0.230053   E    
0693    2MASX J13081765+3323553            9.3    16.97   0.253353   E    
0694    2MASX J10093426+4442382            9.2    15.54   0.145000   E    
0695    2MASX J11413664+6037232            9.2    15.61   0.148656   E    
0696    SDSS J102154.85+072415.5           9.2    17.37   0.290570   SS    
0697    2MASX J12024689+3339546            9.2    17.32   0.286697   E    
0698    2MASX J15001950+2122108            9.2    15.76   0.153200   E    
0699    2MASX J15153188+3603423            9.2    17.25   0.278323   E    
0700    2MASX J11323483+1737192            9.2    17.45   0.299374   E    
0701    2MASX J22222308+1334155            9.2    16.44   0.194208   E    
0702    2MASX J11010708+5117185            9.2    16.49   0.210598   E    
0703    2MASX J13110210+4459564            9.2    16.76   0.232456   E    
0704    2MASX J03460305+0100064            9.2    16.44   0.186147   SS    
0705    LCSB S1598N                        9.2    15.71   0.153825   E    
0707    2MASX J11304267+1538467            9.2    17.48   0.298136   Epec       
0708    B2 1558+33C                        9.2    17.33   0.283560   E    
0709    2MASX J14590584+6036367            9.2    16.73   0.230939   E    
0710    SDSS J122620.01+194113.0           9.2    16.66   0.220232   E    
0711    2MASX J16313593+2141086            9.2    16.19   0.182152   E    
0712    SDSS J120449.48+371914.0           9.2    16.19   0.185665   E    
0713    2MASX J08265512+1811476            9.2    17.16   0.265543   SS    
0714    2MASX J13361878+3422207            9.2    17.26   0.281910   E    
0715    2MASX J10250160+0402026            9.2    16.55   0.211304   E    
0716    2MASX J23284448+0001338            9.2    17.44   0.292222   E    
0717    2MASX J13301074+3043313            9.2    17.35   0.290604   E    
0718    SDSS J035103.92-053831.3           9.2    17.49   0.286634   E    
0719    2MASX J13265921+2737514            9.2    16.99   0.255000   E    
0720    2MASX J12485902+4523026            9.2    16.81   0.232523   E    
0721    2MASX J08061419+2633381            9.2    17.20   0.269701   E    
0722    2MASX J17071913+2434052            9.2    16.04   0.170742   E    
0723    2MASX J16161196+1325338            9.2    16.41   0.197498   E    
0724    2MASX J11114116+5740427            9.2    16.64   0.222067   E    
0725    2MASX J14291128+1000383            9.2    16.88   0.240693   E    
0726    2MASX J11073008-0027467            9.2    17.24   0.269832   E    
0727    2MASX J10405672+3848277            9.2    17.13   0.266727   E    
0728    2MASX J10444382+2741576            9.2    16.56   0.213886   E    
0729    2MASX J10212903+0428341            9.2    15.75   0.154884   E    
0730    2MASX J10543788+2943390            9.2    16.94   0.246987   E    
0731    2MASX J15025526+1104447            9.2    16.01   0.170222   E    
0732    2MASX J11333022+4619329            9.2    17.15   0.267888   E    
0733    2MASX J10511990+0505323            9.1    16.71   0.224995   E    
0734    2MASX J15335451+1950050            9.1    17.12   0.255048   E    
0735    2MASX J10195762-0159473            9.1    16.69   0.218100   E    
0736    SDSS J123841.49+092832.7           9.1    16.75   0.229968   E    
0737    2MASX J14392434+5122163            9.1    17.44   0.299822   E    
0738    2MASX J16275760+2944378            9.1    17.10   0.261120   E    
0739    2MASX J13550992+3656277            9.1    16.92   0.247276   E    
0740    2MASX J13583975+5922023            9.1    16.82   0.237825   E    
0741    2MASX J12060354+3749018            9.1    16.93   0.246333   E    
0742    2MASX J23293166+1550219            9.1    17.20   0.267118   E    
0743    2MASX J12245540+4157436            9.1    16.98   0.249139   E    
0744    2MASX J10151471+1345171            9.1    17.25   0.271224   E    
0745    2MASX J02431231-0101121            9.1    16.88   0.238614   E    
0746    2MASX J09010648+0747471            9.1    15.75   0.148299   E    
0747    2MASX J09512097+0432330            9.1    17.08   0.257961   E    
0748    2MASX J14013644+1350063            9.1    16.52   0.211605   E    
0749    2MASX J15591044+3826290            9.1    17.36   0.290933   SS    
0750    2MASX J23421059-0958330            9.1    17.29   0.278600   E    
0751    2MASX J12513012+0358038            9.1    16.62   0.216748   E    
0752    2MASX J12100232+1434443            9.1    17.19   0.267723   E    
0753    2MASX J08022926+2325161            9.1    17.28   0.271729   SS    
0754    SDSS J122417.59-021432.3           9.1    17.35   0.287115   E    
0755    SDSS J113800.88+521303.9           9.1    17.41   0.296018   SS     
0756    2MASX J02353346-0928046            9.1    17.14   0.264587   E    
0757    2MASX J02405114-0055564            9.1    16.89   0.239638   E    
0758    2MASX J12045599+5024224            9.1    16.67   0.223239   E    
0759    2MASX J21582783+1132151            9.1    16.98   0.238618   E    
0760    2MASX J16132664+4351299            9.1    16.70   0.227265   E    
0761    2MASX J15122657+0201152            9.1    16.70   0.220486   E    
0762    2MASX J13293009+0039434            9.1    16.62   0.216873   E    
0764    2MASX J07513106+3210071            9.1    17.40   0.280022   E    
0765    2MASX J13045122+4746170            9.1    15.53   0.143429   E    
0766    2MASX J12043514+1105449            9.1    16.72   0.225715   E    
0767    2MASX J13323501-0224038            9.1    16.86   0.236629   E    
0768    2MASX J16322680+2539372            9.1    17.20   0.268991   E    
0769    2MASX J14040023+5750431            9.1    16.96   0.250465   E    
0770    2MASX J09421598+1848031            9.1    16.67   0.221203   E    
0771    2MASX J11032141+5519370            9.1    17.00   0.254439   E    
0772    2MASX J08565652+3711404            9.1    17.41   0.289316   E    
0773    2MASX J15472577+1034177            9.1    16.91   0.238472   E    
0774    2MASX J12354790+1533214            9.1    17.36   0.284631   E    
0775    2MASX J13403264+2240088            9.1    17.14   0.267000   E    
0776    2MASX J10102647+1844273            9.1    16.55   0.210741   E    
0777    2MASX J21184907+0033376            9.1    17.42   0.276486   E    
0778    2MASX J00505806-0929227            9.1    16.42   0.200131   E    
0779    SDSS J094017.12+022504.6           9.1    17.39   0.286238   E    
0780    2MASX J23373975+0016165            9.1    17.30   0.277230   E    
0781    2MASX J12441115+1428566            9.0    17.22   0.271987   E    
0782    2MASX J00274622-1032282            9.0    15.99   0.167162   E    
0783    SDSS J102629.10+094519.7           9.0    17.15   0.262280   Epec      
0784    2MASX J16090942+1625497            9.0    15.61   0.143370   E    
0785    2MASX J22354518-0048156            9.0    17.51   0.297018   E    
0786    2MASX J13203369+3215078            9.0    16.23   0.188113   E    
0787    SDSS J144014.61+034142.0           9.0    17.43   0.291376   E    
0788    2MASX J09524915+5153053            9.0    16.56   0.215108   E    
0789    2MASX J08542169+0449308            9.0    15.83   0.156835   SS     
0790    2MASX J16085807+5418175            9.0    17.09   0.262748   E    
0791    2MASX J12120142+0054253            9.0    17.22   0.271687   E    
0792    2MASX J10233960+0411116            9.0    17.41   0.290600   E       
0793    2MASX J11410570+5114244            9.0    17.27   0.280374   E    
0794    2MASX J12465124+0017498            9.0    14.41   0.089260   E    
0795    2MASX J21532624+0011405            9.0    16.78   0.217000   E    
0796    2MASX J11562002-0012201            9.0    14.87   0.107661   E    
0797    2MASX J12264370+1950524            9.0    16.73   0.223567   E    
0798    2MASX J21512786-0842048            9.0    16.48   0.202465   E    
0799    2MASX J10472505+2309174            9.0    16.19   0.182639   SS    
0800    2MASX J11191739+1419465            9.0    15.57   0.143781   SS    
0801    2MASX J16351505+3756304            9.0    16.71   0.225451   E    
0802    SDSS J102751.31+082528.5           9.0    17.44   0.293734   E    
0803    2MASX J08382529+3017144            9.0    17.46   0.292273   E    
0804    SDSS J135546.07+025455.8           9.0    16.87   0.238890   SS    
0805    2MASX J14450902+5958005            9.0    17.23   0.276812   E    
0806    2MASX J11302955+3320517            9.0    16.68   0.222623   E    
0807    2MASX J01260943-1018236            9.0    16.98   0.246929   E    
0808    2MASX J11331676+5307439            9.0    17.01   0.254172   E    
0809    2MASX J11571349+1709108            9.0    17.36   0.278793   E    
0810    2MASX J10490679+3434458            9.0    17.41   0.293138   E    
0811    2MASX J08410559+3831588            9.0    16.99   0.246208   E    
0812    2MASX J14415258+2633013            9.0    16.75   0.228200   E    
0813    2MASX J09060463+1106359            9.0    16.05   0.172493   E    
0814    SDSS J085650.30+032144.7           9.0    17.41   0.287476   E    
0815    SDSS J170041.75+641258.7           9.0    16.70   0.224000   E    
0816    2MASX J13253911+5037556            9.0    16.95   0.248733   E    
0817    2MASX J09062818+0345349            9.0    16.47   0.203415   E    
0818    2MASX J13370466+2057491            9.0    16.29   0.190467   E    
0819    2MASX J14423274+0747024            9.0    16.01   0.169048   E    
0820    2MASX J11430832+3455136            9.0    16.05   0.174067   E    
0821    SDSS J111811.48+271207.1           9.0    17.36   0.288121   E    
0822    2MASX J13242050+1256522            9.0    17.20   0.268998   E    
0823    2MASX J13460350+0309312            9.0    16.80   0.231805   E    
0824    2MASX J14264096+2408467            9.0    15.61   0.144863   E    
0825    UGC 10110                          9.0    14.13   0.077277   E    
0826    2MASX J08374604+1952086            9.0    16.75   0.226355   E    
0827    2MASX J00523376-0930085            9.0    17.29   0.276948   E    
0828    2MASX J14295396+4517311            9.0    16.45   0.205522   E    
0829    2MASX J12433534+2935021            9.0    16.90   0.242720   E    
0830    SDSS J141754.96+270434.4           9.0    15.79   0.157569   SS    
0831    2MASX J12374155-0121377            9.0    15.77   0.155111   E    
0832    2MASX J09065771+4607471            9.0    15.91   0.165000   E    
0833    2MASX J13545624+0430469            9.0    17.33   0.281700   E    
0834    2MASX J17284817+6107301            9.0    16.99   0.247970   E    
0835    2MASX J09514352+0444466            9.0    16.46   0.202365   E    
0836    SDSS J225630.04-003210.8           9.0    16.81   0.223788   E    
0837    SDSS J154105.61+073232.7           9.0    17.39   0.281255   E    
0838    2MASX J12170158+1429300            9.0    16.95   0.243164   E    
0839    2MASX J09203791+5807157            8.9    17.34   0.282460   E    
0840    2MASX J07465905+2738197            8.9    17.02   0.248387   E    
0841    2MASX J08290920+3227314            8.9    17.35   0.278370   E    
0842    LCRS B125223.9-030424              8.9    16.72   0.225113   E    
0843    ZwCl 1700.5+3322 d                 8.9    14.36   0.086405   E    
0844    2MASX J12493954+5827430            8.9    16.37   0.198708   E    
0845    2MASX J22311324-0926318            8.9    17.10   0.252069   E    
0846    2MASX J16193457+3827582            8.9    16.18   0.184205   E    
0847    2MASX J10111410+2555060            8.9    16.92   0.241979   E    
0848    2MASX J01300545-0822021            8.9    16.87   0.237972   E    
0849    2MASX J01032601+1526251            8.9    17.14   0.246136   E    
0850    2MASX J11222711+2511247            8.9    17.04   0.255000   E    
0851    2MASX J15051642+0527036            8.9    16.79   0.226646   E    
0852    2MASX J11331779+1919483            8.9    16.55   0.209884   E    
0853    2MASX J11150160+4233412            8.9    17.46   0.297629   E    
0854    2MASX J01011922-0003189            8.9    16.35   0.193522   E    
0855    2MASX J16494120+3300186            8.9    17.25   0.273375   E    
0856    LCRS B103920.2-022044              8.9    16.71   0.215080   E    
0857    2MASX J11234552+3717347            8.9    17.15   0.264398   E    
0858    2MASX J08530416+1952080            8.9    17.28   0.276649   E    
0859    2MASX J12032293+0448035            8.9    15.92   0.164988   E    
0860    2MASX J11205811+3347418            8.9    16.88   0.236470   E    
0861    2MASX J16401981+4642409            8.9    16.72   0.224351   E    
0862    2MASX J22012068+1208451            8.9    16.49   0.193552   E    
0863    2MASX J10560602+1451502            8.9    17.48   0.298398   E    
0864    2MASX J16233751+2144246            8.9    15.79   0.152573   E    
0865    2MASX J12291026+1443430            8.9    17.39   0.285505   E    
0866    2MASX J14422988+2945487            8.9    16.60   0.215343   E    
0867    2MASX J12572755+5140414            8.9    17.42   0.295195   E    
0868    2MASX J08104775+0905350            8.9    15.96   0.167277   E    
0869    2MASX J21574072+0109485            8.9    16.71   0.216550   E    
0870    2MASX J15104086+1538122            8.9    15.13   0.119057   E    
0871    2MASX J09264567+3642584            8.9    16.92   0.244032   E    
0872    2MASX J17202828+5555222            8.9    17.27   0.274393   E       
0873    IC 2402                            8.9    13.80   0.067373   E    
0874    2MASX J10594338+1307191            8.9    17.37   0.288278   E    
0875    2MASX J12324079+4621528            8.9    16.85   0.236682   E    
0876    2MASX J12261643+3158090            8.9    16.05   0.173297   E    
0877    2MASX J12350687-0051327            8.9    14.92   0.109239   E    
0878    2MASX J08455957+2308006            8.9    16.75   0.225462   E    
0879    2MASX J10442272-0017514            8.9    16.63   0.213006   E    
0880    2MASX J14474060+2016204            8.9    16.34   0.190910   E    
0881    2MASX J12441204+4030267            8.9    16.52   0.209221   E    
0882    2MASX J09202854+4200364            8.9    17.49   0.299998   E    
0883    2MASX J13202990+3621049            8.9    17.14   0.266011   E    
0884    2MASX J12361934+2827170            8.9    16.75   0.227555   E    
0885    SDSS J121325.92+212257.4           8.9    16.74   0.223656   E    
0886    2MASX J10080912+6012123            8.9    16.82   0.234460   E    
0887    2MASX J09174310+0047466            8.8    16.42   0.197942   E    
0888    2MASX J08042135+4647136            8.8    16.34   0.186882   E    
0889    2MASX J08250928+2634381            8.8    17.00   0.244547   G      
0890    2MASX J11514620+2832448            8.8    17.17   0.265106   E    
0891    2MASX J01354896-1012315 NED01      8.8    16.03   0.170874   E    
0892    SDSS J095543.25+111715.9           8.8    17.51   0.299029   Epec      
0893    2MASX J09352743+0730257            8.8    16.67   0.215999   E    
0894    2MASX J14534973+2742154            8.8    16.77   0.227434   E    
0895    2MASX J08414561+3124125            8.8    17.39   0.282496   E    
0896    2MASX J16552596+3004237            8.8    16.95   0.242039   E    
0897    2MASX J15545773+3415002            8.8    16.33   0.191981   E    
0898    2MASX J14492025-0139362            8.8    17.23   0.264994   E    
0899    SDSS J112916.81-004244.3           8.8    17.35   0.282049   E    
0900    2MASX J13362989+5539564            8.8    16.72   0.226500   E    
0901    2MASX J14422611+1254168            8.8    15.19   0.121058   E    
0902    2MASX J23591456+1351308            8.8    17.04   0.247131   Epec      
0903    2MASX J12050921+5856343            8.8    15.28   0.126784   E    
0904    2MASX J01002508-1052417            8.8    16.59   0.210914   E    
0905    2MASX J15380514+1217557            8.8    16.81   0.227723   E    
0906    LCRS B114758.3-030229              8.8    17.20   0.266501   E    
0907    2MASX J11045557+4725159            8.8    16.66   0.218802   E    
0908    MCG +09-15-062                     8.8    14.34   0.085906   E    
0909    2MASX J14381016+5030122            8.8    16.98   0.246695   SS    
0910    2MASX J10391433+6122042            8.8    15.64   0.148050   E    
0911    2MASX J14053652+0132396            8.8    16.16   0.178093   E    
0912    2MASX J09235735+1522569            8.8    16.16   0.179640   E    
0913    2MASX J01040443-0026042            8.8    17.35   0.279122   E    
0914    2MASX J11441407+4343165            8.8    16.86   0.236213   E    
0915    2MASX J10145267+2149018            8.8    15.93   0.164057   E    
0916    SDSS J125641.74+444852.8           8.8    17.48   0.298079   E    
0917    2MASX J15161794+0005203            8.8    15.25   0.120790   E    
0918    2MASX J13184290+3843000            8.8    16.83   0.234774   E    
0919    2MASX J10073422+2007379            8.8    17.09   0.255077   E    
0920    2MASX J12375962+4243484            8.8    17.41   0.288280   E    
0921    2MASX J15210797+1847572            8.8    16.95   0.235170   E    
0922    2MASX J07582902+2639492            8.8    16.91   0.234718   E    
0923    SDSS J145555.32+165746.4           8.8    17.42   0.289000   E    
0924    2MASX J09342510+3136498            8.8    15.27   0.125824   E    
0925    LCRS B121150.6-031751              8.8    16.17   0.177900   E    
0926    2MASX J10304263+0418219            8.8    15.93   0.161110   SS    
0927    SDSS J101924.91+074629.5           8.8    17.50   0.298291   E    
0928    2MASX J12374668+4812273            8.8    17.24   0.272592   SS    
0929    2MASX J12251461+6121587            8.8    17.36   0.284769   E     
0930    2MASX J09195065+3550454            8.8    16.69   0.221563   E    
0931    2MASX J08151743+2750334            8.8    17.34   0.280434   E    
0932    2MASX J11451666+3451000            8.8    17.26   0.273928   E    
0933    2MASX J12120883+1347328            8.8    16.11   0.174488   E    
0934    2MASX J13220241+3643512            8.8    16.14   0.179849   E    
0935    UGC 08669 NED01                    8.8    14.04   0.075732   E    
0936    2MASX J00241023-0027461            8.8    17.14   0.260961   E    
0937    2MASX J09175344+5144009            8.8    16.73   0.224992   E    
0938    2MASX J15474400+0310542            8.8    17.28   0.254468   E    
0939    2MASX J08433232+4132143            8.7    17.10   0.255258   E    
0940    2MASX J15123469+1628385            8.7    16.29   0.187219   E    
0941    2MASX J07575811+3939093            8.7    17.15   0.256401   E    
0943    2MASX J10250685+3251250            8.7    16.89   0.238923   E     
0944    MCG -02-02-086                     8.7    13.39   0.055672   E    
0945    2MASX J11304467+1915526            8.7    15.77   0.153474   E    
0946    2MASX J10511031+0903572            8.7    16.71   0.221194   E    
0947    2MASX J13254371+2802335            8.7    17.04   0.252690   E    
0948    2MASX J12375307+3446313            8.7    16.72   0.224910   E    
0949    2MASX J12043869+6549513            8.7    16.50   0.205393   E    
0950    2MASX J15531761+1019087            8.7    16.83   0.226401   E    
0951    2MASX J13404035+6728045            8.7    16.96   0.245174   E    
0952    2MASX J11542338+5003156            8.7    17.39   0.287819   E    
0953    SDSS J151835.47+181441.1           8.7    16.34   0.186440   E    
0954    2MASX J12505826+0903205            8.7    17.50   0.298000   E    
0955    2MASX J08432083+3920404            8.7    17.50   0.296084   E    
0956    2MASX J10232175+5018290            8.7    15.73   0.152003   E    
0957    2MASX J11534498+1521223            8.7    15.02   0.111987   E    
0958    2MASX J15055031+0429097            8.7    16.72   0.217724   E    
0960    2MASX J09273277+0145370            8.7    15.79   0.148636   E    
0961    2MASX J10345428+1214553            8.7    16.30   0.188518   E    
0962    SDSS J141756.67+254326.2           8.7    16.87   0.236299   G       
0963    2MASX J01131052+1409353            8.7    17.55   0.298137   E    
0964    2MASX J13470927+2126084            8.7    16.41   0.197291   E    
0965    2MASX J12572122+1348250            8.7    16.72   0.220733   E    
0966    2MASX J12164544+4514098            8.7    17.07   0.256687   E    
0967    2MASX J10274425+1125116            8.7    16.92   0.238921   E    
0968    2MASX J09312816+4424163            8.7    16.69   0.219191   SS    
0969    2MASX J12542979+2545015            8.7    16.79   0.230860   E    
0970    2MASX J11111122+0045078            8.7    16.29   0.184769   E    
0971    VII Zw 579                         8.7    15.84   0.158645   E     
0973    2MASX J13412783+2851280            8.7    17.46   0.294948   Epec       
0974    2MASX J11290694+0233070            8.7    17.15   0.259603   E    
0975    2MASX J11410001+3848078            8.7    17.21   0.267567   SS    
0976    SDSS J142751.43-023634.5           8.7    17.41   0.278939   E    
0977    2MASX J01445054-0839250            8.7    16.33   0.190295   E    
0978    2MASX J13261760+0013177            8.7    14.28   0.082700   E    
0979    2MASX J10542755+3109288            8.7    17.08   0.252318   E    
0980    SDSS J122658.76+183059.1           8.7    15.18   0.119713   E    
0981    SDSS J104302.00+093057.4           8.7    17.29   0.274097   E    
0982    SDSS J165807.85+383716.5           8.7    17.10   0.257912   E    
0983    SDSS J153618.97+452246.8           8.7    16.85   0.236206   SS    
0984    SDSS J133737.88+494015.6           8.7    17.23   0.272440   SS    
0985    2MASX J16161685+1623381            8.7    17.52   0.292913   E    
0986    2MASX J08382280+4617125            8.7    17.24   0.270598   E    
0987    SDSS J094801.18+290011.4           8.7    16.61   0.213734   E    
0988    2MASX J13054048+1059513            8.7    16.10   0.173740   E    
0989    2MASX J13334790+4905166            8.7    17.30   0.281024   E    
0990    2MASX J16303309+3316198            8.7    17.41   0.287852   E    
0991    SDSS J132318.72+060800.9           8.7    17.47   0.291153   E    
0992    2MASX J12493763+5127149            8.7    17.38   0.286842   E    
0993    2MASX J15152280+2034103            8.7    17.00   0.243073   E    
0994    2MASX J09551976+0954146            8.7    16.49   0.200217   E    
0995    2MASX J14440406+2029072            8.7    17.03   0.248222   SS    
0996    2MASX J17042839+3414548            8.7    16.90   0.237910   E    
0997    2MASX J13420697+4725526            8.7    16.08   0.172175   E    
0998    2MASX J11570606+1629358            8.7    17.44   0.277831   E    
0999    2MASX J11565195+0755148            8.7    17.50   0.299376   E    
1000    2MASX J21340602-0031209            8.7    16.85   0.229203   E    
1001    CGCG 162-041                       8.7    14.07   0.075926   E    
1002    2MASX J10535662+5909155            8.7    16.40   0.198533   SS    
1003    2MASX J10064015+2140145            8.7    16.33   0.189080   E    
1004    2MASX J09340989+0418342            8.7    16.99   0.242855   E    
1005    2MASX J10400856+1633227            8.7    16.21   0.178998   E    
1006    SDSS J133232.95+502502.4           8.7    17.24   0.272861   E    
1007    SDSS J115553.35+070123.3           8.7    17.45   0.293654   E    
1008    2MASX J15270858+5018174            8.6    17.32   0.278007   E    
1009    2MASX J09581235+2346452            8.6    15.66   0.145129   E    
1010    2MASX J12110427-0151573            8.6    16.93   0.240329   E    
1011    2MASX J11401183+1241314            8.6    17.31   0.274126   E    
1012    2MASX J16031902+0316442            8.6    16.97   0.222175   E    
1013    2MASX J15332896+2348362            8.6    16.85   0.227503   E    
1014    2MASX J11312172+2126275            8.6    15.45   0.134283   E    
1015    2MASX J07464082+2217035            8.6    17.23   0.257722   E    
1016    2MASX J23373759-0040399            8.6    17.43   0.287492   E    
1017    2MASX J14055748+4125287            8.6    17.24   0.271236   E    
1018    SDSS J080520.11+102751.4           8.6    17.42   0.288503   E      
1019    2MASX J13172766+0218441            8.6    17.49   0.294702   E     
1021    2MASX J03174605-0625427            8.6    16.40   0.189752   E    
1022    2MASX J02243325-0731115            8.6    17.34   0.277114   E    
1023    2MASX J09254889+0745051            8.6    16.12   0.172306   SS    
1024    2MASX J10241900+3114320            8.6    16.98   0.244699   E    
1025    2MASX J13485338+0756478            8.6    17.04   0.249579   E    
1026    2MASX J15094143+2924497            8.6    15.48   0.135070   E    
1027    2MASX J15533786+2422557            8.6    16.57   0.204843   E    
1028    2MASX J09364994+1028244            8.6    17.27   0.269766   E    
1029    2MASX J15485481+1701322            8.6    17.45   0.287831   E      
1030    2MASX J12325977+2249453            8.6    16.68   0.218693   E    
1031    2MASX J23542893-0842184            8.6    17.40   0.282742   E    
1032    2MASX J11320623+4446169            8.6    16.60   0.211778   E    
1033    2MASX J09015026+3818032            8.6    16.32   0.189440   E    
1034    2MASX J16045379+4450329            8.6    16.84   0.233515   E    
1036    2MASX J15472810+1249455            8.6    16.19   0.176734   E    
1037    2MASX J16383832+4636472            8.6    15.46   0.135127   E    
1038    SDSS J141208.09+282214.8           8.6    16.77   0.226297   E    
1039    2MASX J15112917+1439390            8.6    16.22   0.179791   E    
1040    2MASX J14552102+0410594            8.6    16.78   0.222065   E    
1041    2MASX J15492872+2356093            8.6    16.66   0.211559   E    
1042    2MASX J15002251+5218283            8.6    17.34   0.279818   E    
1043    2MASX J10454851+0420320            8.6    15.83   0.153897   E    
1044    2MASX J10495844+1649215            8.6    17.29   0.273635   E    
1045    SDSS J105306.18+085932.6           8.6    16.02   0.166468   E    
1046    2MASX J09362208+3906291            8.6    17.36   0.283019   SS    
1047    2MASX J12084935+0657057            8.6    16.91   0.239206   E    
1048    2MASX J10562944+1441536            8.6    17.52   0.298941   E    
1049    2MASX J12072605+6321032            8.6    16.95   0.242083   E    
1050    2MASX J21443458+0108218            8.6    16.86   0.226793   E    
1051    2MASX J09082483+0603567            8.6    15.89   0.156465   E    
1052    2MASX J02395459-0042418            8.6    17.54   0.298319   E    
1053    2MASX J21493744+0047486            8.6    17.57   0.288172   E    
1054    2MASX J15421826+4154318            8.6    15.62   0.142427   E    
1055    SDSS J125248.20+040120.4           8.6    16.98   0.241671   E    
1056    SDSS J120050.60-012755.6           8.6    17.24   0.267160   Epec   
1057    2MASX J21423470+1230203            8.6    17.51   0.276983   E    
1058    2MASX J12383963+6413430            8.6    17.18   0.265032   Epec       
1059    2MASX J13024868+4755105            8.6    15.56   0.140616   E    
1060    2MASX J09292663+1936145            8.6    17.51   0.290858   E    
1061    2MASX J11342816+4433064            8.6    17.08   0.253205   E    
1062    4C +10.44                          8.6    16.56   0.202121   E       
1063    2MASX J15182841+0045551            8.5    17.26   0.264230   E    
1064    2MASX J16311044+2328377            8.5    17.03   0.244087   E    
1065    2MASX J12173965+4729229            8.5    17.28   0.273229   E    
1066    2MASX J01045535+0003367            8.5    17.30   0.272000   E    
1067    2MASX J13261255+2153387            8.5    17.28   0.273000   E    
1068    2MASX J08224339+4139592            8.5    16.66   0.211007   E    
1069    2MASX J22161561-0919590            8.5    14.41   0.084058   E    
1070    2MASX J12142101-0218393            8.5    17.48   0.292626   E    
1071    2MASX J15583566+3034586            8.5    17.46   0.288332   E    
1072    LCSB S2059P                        8.5    16.13   0.175980   E       
1073    2MASX J21505471+1134519            8.5    17.44   0.276216   E    
1074    SDSS J114013.22+070916.7           8.5    17.45   0.284617   E    
1075    2MASX J08594812+0411111            8.5    16.61   0.207656   E    
1076    2MASX J15101744+1239261            8.5    16.27   0.182859   E    
1077    2MASX J09050105+4012283            8.5    17.27   0.272123   E    
1078    2MASX J10500871+3130225            8.5    17.17   0.260303   E    
1079    2MASX J10330172+4019233            8.5    15.98   0.166657   E    
1080    SDSS J123146.83+141559.4           8.5    17.52   0.294907   E    
1081    2MASX J01370280+0102599            8.5    17.03   0.245032   E    
1082    2MASX J12123303+0604361            8.5    15.52   0.137074   E    
1084    2MASX J08512644+3558135            8.5    17.29   0.271616   E    
1085    2MASX J09373402+0834152            8.5    15.57   0.137562   E    
1086    2MASX J17161684+5907310            8.5    17.09   0.251360   E    
1087    CGCG 134-067                       8.5    13.72   0.063030   E    
1088    SDSS J140138.37+263527.6           8.5    17.38   0.284036   SS    
1089    2MASX J09591937+4603035            8.5    16.70   0.220883   E    
1090    2MASX J08404913+3008513            8.5    17.53   0.290353   E    
1092    2MASX J08572884+0323490            8.5    16.52   0.199733   E    
1093    SDSS J143300.13+300608.2           8.5    17.21   0.266538   E    
1094    SDSS J163357.99+172839.5           8.5    17.30   0.267114   SS    
1095    SDSS J133235.53+105737.9           8.5    17.56   0.299640   E    
1096    2MASX J13104879+4609353            8.5    16.22   0.183810   E    
1097    2MASX J21425447+1252267            8.5    17.16   0.239913   E    
1098    2MASX J09355479+0636208            8.5    16.78   0.221714   E    
1099    2MASX J12460302+1243469            8.5    16.92   0.237905   E    
1100    2MASX J10475135+0723396            8.5    16.93   0.238080   E    
1101    2MASX J09294016+0803069            8.5    16.71   0.214328   E    
1102    2MASX J12510934+4642401            8.5    17.11   0.257966   E    
1103    2MASX J07285570+4159465            8.5    16.52   0.196669   E    
1104    2MASX J10250881+4150178            8.5    17.20   0.265791   E    
1105    2MASX J11580383+0005545            8.5    17.09   0.253243   E    
1106    2MASX J09451288+2201555            8.5    17.36   0.277802   E    
1107    2MASX J12072497-0150416            8.5    16.59   0.209637   SS    
1108    2MASX J11044865+3212397            8.5    17.04   0.246723   E    
1109    SDSS J112102.85+462451.0           8.5    17.47   0.294350   E    
1110    2MASX J16060156+0856469            8.5    16.41   0.191168   E    
1111    2MASX J08445589+0509070            8.5    16.98   0.238359   E    
1112    CGCG 165-049                       8.5    14.04   0.073968   E    
1113    2MASX J14220686+1613562            8.5    17.23   0.267000   E    
1114    2MASX J08193989+4952348            8.5    15.61   0.139110   E    
1115    2MASX J08491074+3731095            8.5    16.94   0.236657   E    
1117    2MASX J14233818+2218340            8.5    15.48   0.133023   E    
1118    2MASX J12431790+1900486            8.5    15.05   0.113202   E    
1119    2MASX J11300126+1256168            8.5    17.05   0.245474   E    
1120    2MASX J09443444-0044300            8.5    16.61   0.203971   E    
1121    2MASX J13000229+6403010            8.5    17.21   0.266468   E    
1122    2MASX J14564393+5549074            8.5    17.35   0.280366   E    
1123    2MASX J01024546-1004329            8.5    15.78   0.150939   E    
1124    2MASX J13100101+0856003            8.5    17.12   0.255051   E    
1125    2MASX J08261217+2157427            8.5    17.24   0.261513   E    
1126    2MASX J10031223+2118039            8.5    15.72   0.147671   E    
1127    2MASX J13051414+6416170            8.5    16.46   0.199859   E    
1128    SDSS J075137.20+325447.4           8.5    16.69   0.207900   E    
1129    2MASX J12364945+0541262            8.5    16.43   0.196902   E    
1130    2MASX J09453105+0946342            8.5    16.73   0.219610   E    
1131    2MASX J09211358+0456446            8.4    17.25   0.262574   E    
1132    2MASX J12262278+5549193            8.4    17.42   0.287461   E    
1133    SDSS J022828.37-005445.8           8.4    17.58   0.299980   E    
1134    2MASX J11092205+2355065            8.4    16.29   0.187000   E    
1135    SDSS J143343.41+514316.5           8.4    17.27   0.273815   E    
1136    4C +14.67                          8.4    17.41   0.279130   E    
1137    LCSB S1701N                        8.4    17.08   0.249252   E    
1138    2MASX J10343030+1234502            8.4    16.26   0.182837   E    
1139    2MASX J09552918+3600294            8.4    16.25   0.185003   E    
1140    2MASX J15501392+1547440            8.4    15.68   0.144196   E     
1141    SDSS J105024.70-012057.3           8.4    17.55   0.293900   E      
1142    2MASX J17205839+5556212            8.4    16.86   0.230248   E    
1143    2MASX J12365883+0438172            8.4    17.00   0.244100   E    
1144    SDSS J100829.29+405854.8           8.4    17.39   0.284275   E      
1145    2MASX J12125909+2727050            8.4    16.20   0.179652   E    
1146    2MASX J08431902+3159580            8.4    17.53   0.293822   E    
1148    2MASX J12460411+1649439            8.4    16.93   0.237106   E    
1149    CGCG 435-044                       8.4    14.15   0.075440   E    
1150    2MASX J15125926+0013410            8.4    16.83   0.222970   E    
1151    B2 0836+29                         8.4    14.28   0.079058   E    
1152    2MASX J15091716+1402255            8.4    16.82   0.225278   E     
1153    2MASX J13191125+4155548            8.4    16.46   0.200145   E    
1154    2MASX J13283719+4412562            8.4    17.32   0.276487   E    
1155    SDSS J113903.18+423717.8           8.4    16.16   0.176278   E    
1156    2MASX J08003599+1532199            8.4    16.44   0.194889   E    
1157    2MASX J22250245+0033070            8.4    16.52   0.195568   E    
1158    2MASX J08503365+3631137            8.4    17.42   0.282754   E    
1159    2MASX J10151704+0257168            8.4    17.02   0.243716   E    
1160    2MASX J16474406+2956314            8.4    14.84   0.100796   E    
1161    2MASX J12420834+0503192            8.4    17.14   0.257001   E    
1162    2MASX J15582770-0032350            8.4    16.12   0.156737   E    
1163    SDSS J162437.30+114704.5           8.4    17.62   0.296000   E    
1164    2MASX J10245098+0621035            8.4    17.25   0.268053   E    
1165    2MASX J11050976+0942093            8.4    16.76   0.222236   E    
1166    2MASX J22295446-0921345            8.4    17.43   0.279639   SS    
1167    2MASX J09155785+0529007            8.4    15.67   0.143263   E    
1168    SDSS J092421.98-005103.8           8.4    17.35   0.275757   E    
1169    2MASX J11534215+1424403            8.4    16.06   0.166781   E    
1171    SDSS J115928.74+043822.8           8.4    17.37   0.280558   E    
1172    2MASX J10502789+1654102            8.4    17.52   0.294317   E    
1174    2MASX J11310763+0224271            8.4    17.16   0.257493   Epec        
1175    SDSS J095952.69+451303.1           8.4    17.43   0.288691   E    
1177    2MASX J15352172+3723454            8.4    15.81   0.153674   E    
1178    2MASX J23420919+1527297            8.4    17.37   0.274250   E    
1179    2MASX J14023302+1408235            8.4    17.01   0.246213   E    
1180    2MASX J15355766+3837202            8.4    17.31   0.274855   E    
1181    2MASX J13252972+4855405            8.4    17.39   0.286593   E    
1182    2MASX J00495939-0853413            8.4    15.26   0.121848   SS  
1183    2MASX J12180837+3631035            8.4    16.93   0.237830   E    
1184    SDSS J134932.29+005544.3           8.4    17.42   0.283679   E    
1185    2MASX J14420196+3919511            8.4    16.22   0.182395   E    
1186    2MASX J12130807+1201113            8.4    15.71   0.146880   E    
1187    2MASX J11510057+1324272            8.4    16.76   0.220749   E    
1188    2MASX J14393169+1027224            8.4    16.88   0.231797   E    
1189    2MASX J15111936+0145169            8.4    16.80   0.220228   E    
1190    2MASX J14205547+3513480            8.4    16.36   0.191290   E    
1191    SDSS J153740.64+495446.0           8.4    17.54   0.298179   E    
1192    2MASX J13530637+0508586            8.4    14.21   0.078828   E    
1193    VPC 0922                           8.4    14.63   0.093598   E    
1194    SDSS J093651.08+245730.7           8.4    16.76   0.223123   E    
1195    2MASX J12134664-0209544            8.4    16.18   0.176705   E    
1196    SDSS J154950.91+234444.1           8.4    17.27   0.262217   SS    
1197    2MASX J16044607+5238220            8.4    16.71   0.219750   E    
1198    2MASX J22262914+1304177            8.4    15.57   0.132293   E    
1199    SDSS J092709.29+084952.6           8.4    17.58   0.295018   E    
1200    2MASX J02413204-0047358            8.4    16.16   0.174547   E    
1201    2MASX J16264388+0850076            8.4    17.06   0.241972   E    
1203    SDSS J095012.14+052617.2           8.4    17.14   0.254971   E    
1204    2MASX J22132500-0928540            8.4    17.46   0.282167   E    
1205    LCRS B104314.0-023900              8.4    16.61   0.206200   E    
1206    2MASX J13274630+3527562            8.4    16.81   0.229242   E    
1207    2MASX J11545005+6040007            8.4    16.95   0.239292   E    
1208    2MASX J11535280-0137384            8.4    17.36   0.278093   E    
1209    2MASX J01020815-1043324            8.4    16.35   0.188594   E    
1210    2MASX J13303064+0515362            8.4    16.11   0.171105   E    
1211    2MASX J09403069+6108327            8.4    17.39   0.280961   E    
1212    2MASX J14064115+5113419            8.4    17.21   0.264539   E    
1213    SDSS J130133.60+351504.0           8.4    17.48   0.293667   E    
1214    2MASX J13295469+2844224            8.4    17.32   0.276701   E    
1215    2MASX J15345783+5438160            8.4    17.34   0.277307   E    
1216    2MASX J11220667+1205524            8.4    16.97   0.238853   E    
1217    2MASX J13015254+6410001            8.3    17.26   0.269141   E    
1218    2MASX J11571104-0135548            8.3    17.44   0.287283   E    
1219    2MASX J09145256+1544322            8.3    14.53   0.089328   E    
1220    2MASX J08164326+4702216            8.3    17.58   0.295350   SS    
1221    2MASX J02114830+0016401            8.3    17.54   0.294901   E    
1222    2MASX J07440004+2145184            8.3    17.19   0.254359   E    
1223    2MASX J03492724-0648159            8.3    17.62   0.283674   E    
1224    2MASX J10383663+0117493            8.3    15.42   0.128526   E    
1225    2MASX J13465790+3012452            8.3    17.51   0.295489   E    
1226    2MASX J13075740+1650483            8.3    16.24   0.181585   E    
1227    2MASX J13364638+1241458            8.3    17.38   0.279057   E    
1228    2MFGC 11354                        8.3    16.92   0.238941   E+S      
1229    2MASX J08574977+0135301            8.3    17.44   0.281321   G      
1230    2MASXi J2219118-090122             8.3    16.97   0.233441   E      
1231    2MASX J09123995+4933561            8.3    16.91   0.236106   E    
1232    2MASX J12485255+4105562            8.3    15.84   0.155572   E    
1233    2MASX J12255652+2736357            8.3    16.62   0.209833   E    
1234    2MASX J14333244+0409243            8.3    15.90   0.156802   E    
1235    2MASX J14054634+4724365            8.3    17.04   0.247217   E    
1236    2MASX J15193632+3134493            8.3    17.55   0.299282   E    
1237    2MASX J14021688+1728568            8.3    16.31   0.185448   E    
1238    2MASX J15554264+2008117            8.3    16.68   0.209214   E    
1239    SDSS J145608.63+380038.5           8.3    17.39   0.283560   G       
1240    2MASX J15565432+2440087            8.3    16.29   0.178691   E    
1241    2MASX J11300108+3302005            8.3    16.72   0.219121   E    
1242    2MASX J13393342+1443578            8.3    17.42   0.281806   E    
1243    2MASX J16141764+2804054            8.3    17.61   0.297903   E    
1244    2MASX J07501945+2301260            8.3    17.18   0.249292   E    
1245    2MASX J02354663-0742506            8.3    17.22   0.261654   G      
1246    2MASX J09330730+1336493            8.3    15.47   0.131215   E    
1247    IC 2938                            8.3    14.28   0.080336   E    
1248    2MASX J11595215+5532053            8.3    14.25   0.080849   E    
1249    2MASX J11513833+2442168            8.3    17.36   0.278738   E    
1250    2MASX J12321515+1021195            8.3    16.04   0.165920   SS    
1251    2MASX J11532766+4433556            8.3    17.40   0.283290   E    
1252    MCG +07-16-007                     8.3    14.53   0.087433   E    
1253    2MASX J10582366+5647417            8.3    15.48   0.135097   E    
1254    2MASX J14035478+3815495            8.3    16.56   0.208522   E    
1255    2MASX J11235159+2238395            8.3    17.16   0.259000   E    
1256    2MASX J16154155+2057530            8.3    17.00   0.229496   E    
1257    2MASX J11552575+1617474            8.3    16.07   0.167367   E    
1258    2MASX J11321201+3934430            8.3    17.58   0.296371   E    
1259    2MASX J14090134+2743362            8.3    16.89   0.233768   E    
1260    2MASX J11402810+5219099            8.3    17.48   0.292676   E    
1262    2MASX J12392473+5617441            8.3    17.06   0.249634   E    
1263    2MASX J14125215+2753181            8.3    15.60   0.140461   E    
1264    2MASX J23541371-1025084            8.3    14.23   0.077691   E    
1265    2MASX J09551240+5034061            8.3    16.65   0.213179   E    
1266    2MASX J16084346+2443376            8.3    17.36   0.266000   E    
1267    2MASX J14292111+2306296            8.3    15.52   0.134784   E    
1268    2MASX J12005393+4800076            8.3    17.37   0.278617   SS  
1269    2MASX J13340753+6440341            8.3    17.02   0.243756   E    
1270    SDSS J125157.99+305422.3           8.3    16.85   0.230703   SS    
1271    MCG +07-27-039                     8.3    14.00   0.072310   E    
1272    SDSS J124856.29+061126.1           8.3    17.56   0.297885   E    
1273    2MASX J07380615+2823592            8.3    16.92   0.231010   SS  
1275    2MASX J14480088+0950489            8.3    16.02   0.166099   E    
1276    2MASX J00320841+1430152            8.3    16.86   0.222649   E+S?    
1277    2MASX J14353849+2055085            8.3    16.14   0.172047   E    
1278    2MASX J16264251+4240120            8.3    16.30   0.187096   E    
1279    2MASX J03120845-0707404            8.3    16.97   0.229446   E    
1280    SDSS J092928.60+042413.3           8.3    17.34   0.269688   E    
1281    2MASX J11112439+1408508            8.3    16.75   0.221157   E    
1282    2MASX J17163513+2835001            8.3    17.43   0.280182   E    
1283    2MASX J13000272+4410016            8.3    17.32   0.274626   E    
1284    2MASX J11572877+3258340            8.3    16.88   0.231338   E    
1285    2MASX J11193313+6317159            8.3    15.80   0.153358   E    
1286    2MASX J10575465+4348423            8.3    16.77   0.224436   E    
1287    2MASX J07404205+4332412            8.3    16.26   0.178350   SS    
1288    2MASX J11443479+6813061            8.3    17.41   0.285668   E    
1289    2MASX J16400236+4123262            8.3    15.88   0.158330   E    
1290    2MASX J13553347+5156181            8.3    17.33   0.276674   E    
1291    SDSS J090317.22-000758.9           8.3    17.59   0.297412   SS    
1292    SDSS J150319.66+044359.1           8.3    17.60   0.298150   E    
1293    2MASX J12492667+2830507            8.3    16.96   0.240358   E    
1294    2MASX J03475821+0058298            8.3    16.73   0.184486   E    
1295    2MASX J08283169+3548283            8.3    17.46   0.282511   E    
1296    2MASX J08004232+3923175            8.3    17.20   0.255359   E    
1297    2MASX J12290616+3437102            8.3    17.35   0.277395   E    
1298    2MASX J09232386+0840365            8.3    15.50   0.130087   E    
1299    2MASX J13353587+4453204            8.3    17.08   0.250288   E    
1300    2MASX J10414368+1440004            8.3    16.40   0.191346   E    
1301    2MASX J09552440+2120039            8.3    17.09   0.246999   E    
1302    2MASX J14374380-0018579            8.3    15.60   0.138023   E    
1303    2MASX J15050196+5536012            8.3    16.51   0.201933   E    
1304    2MASX J16014061+2718161            8.3    16.06   0.164554   SS  
1305    2MASX J15021801+2700308            8.3    17.36   0.273000   E      
1306    2MASX J14222648+4028513            8.2    17.31   0.275985   E    
1307    2MASX J15255324+2827326            8.2    15.79   0.150210   E    
1308    2MASX J22121037-0729156            8.2    16.78   0.215374   E    
1309    SDSS J111201.29+045117.0           8.2    16.91   0.225215   E    
1310    2MASX J13203239+5126421            8.2    17.35   0.277550   E    
1311    2MASX J00532329+1415119            8.2    17.03   0.236547   E    
1312    SDSS J143447.86+020228.6           8.2    17.42   0.280115   SS    
1313    2MASX J11314774+0839311            8.2    16.88   0.227005   E    
1314    2MASX J16313787+4543445            8.2    17.19   0.262740   E    
1315    2MASX J16054041+1625458            8.2    15.53   0.133540   E    
1316    SDSS J112810.38+010153.7           8.2    17.56   0.295034   E    
1317    2MASX J11440681+0547530            8.2    14.85   0.102779   E    
1318    2MASX J09512250+5437137            8.2    16.61   0.211256   E    
1319    2MASX J12242967+3209378            8.2    16.75   0.220293   E    
1320    2MASX J12103898+5138471            8.2    17.44   0.285708   E    
1321    2MASX J12280218+3440397            8.2    17.34   0.277454   E    
1323    SDSS J112928.74+025549.9           8.2    17.01   0.239698   SS      
1324    SDSS J091011.54+013903.7           8.2    17.44   0.284163   E    
1325    2MASX J15234812+0534436            8.2    16.23   0.176079   E    
1326    2MASX J15095786+3644200            8.2    16.09   0.170662   E    
1327    2MASX J08522163+3028556            8.2    17.47   0.285499   E    
1328    2MASX J15284227+0119519            8.2    15.16   0.114202   E    
1329    2MASX J16273931+3002239            8.2    17.20   0.259761   SS    
1330    SDSS J142333.87+023825.2           8.2    17.44   0.282958   E    
1331    2MASX J11533090-0144047            8.2    15.54   0.136411   E    
1332    LCRS B115947.6-031025              8.2    17.22   0.261093   E    
1333    2MASX J13520882+0405455            8.2    17.19   0.258247   E    
1334    2MASX J11080613+0016537            8.2    16.58   0.203493   E    
1335    2MASX J16024697+4528397            8.2    16.64   0.211590   E    
1336    SDSS J092049.70+024513.9           8.2    17.46   0.284133   E    
1337    SDSS J093921.25+260709.8           8.2    17.34   0.275110   SS    
1338    2MASX J07573589+3555285            8.2    17.55   0.290457   E    
1339    2MASX J09563073+0729439            8.2    16.18   0.174087   E    
1340    2MASX J14460307+6406282            8.2    15.11   0.114707   E    
1341    CGCG 018-111 NED01                 8.2    13.46   0.055572   E     
1342    2MASX J08521402+1505131            8.2    16.59   0.204782   E    
1344    2MASX J08280587+4446005            8.2    15.71   0.145029   E    
1345    2MASX J09451948+1005053            8.2    16.73   0.218260   E    
1346    2MASX J11374907+4147427            8.2    17.19   0.258676   E    
1347    2MASX J02211146-0926470            8.2    15.97   0.161337   E    
1349    2MASX J10400653+1037559            8.2    16.94   0.234646   E    
1350    2MASX J10442897+5335474            8.2    17.06   0.248912   E    
1351    2MASX J00423814+1531049            8.2    17.19   0.249188   E    
1352    SDSS J101603.97+303747.9           8.2    17.13   0.252016   SS    
1353    2MASX J15072317+4244030            8.2    16.72   0.217626   E    
1354    2MASX J14483142+2358508            8.2    15.28   0.119306   E    
1355    2MASX J08514169+1636544            8.2    16.22   0.179355   E    
1356    2MASX J10191631+3127510            8.2    17.46   0.285484   E    
1357    2MASX J02123082-0018107            8.2    17.14   0.252790   E      
1358    2MASX J14234736+3511119            8.2    16.42   0.193242   E    
1359    2MASX J12122536+3942507            8.2    17.24   0.263281   E    
1361    MCG +09-26-045                     8.2    14.93   0.107175   E    
1362    2MASX J10203038+3922117            8.2    15.72   0.147602   E    
1363    2MASX J07480983+2722232            8.2    16.56   0.201305   E    
1364    2MASX J11535667+6030196            8.2    14.96   0.107511   E    
1365    2MASX J10562290+2710079            8.2    17.01   0.242405   E    
1366    2MASX J16412953+4305072            8.2    17.26   0.267368   E    
1367    2MASX J00470596+1544352            8.2    17.11   0.245247   E    
1368    2MASX J13042719+3335129            8.2    16.32   0.187342   E    
1369    2MASX J17272346+5510538            8.2    17.09   0.247260   E    
1370    2MASX J13292035+4155461            8.2    16.91   0.234931   E    
1371    2MASX J15061443+0334452            8.2    16.87   0.225760   E    
1372    2MASX J13425381+4638427            8.2    17.28   0.266327   E    
1373    2MASX J10310089+5325418            8.2    15.54   0.136341   E    
1374    SDSS J134526.75+134356.4           8.2    15.82   0.151800   E    
1375    2MASX J00155012-1002427            8.2    16.23   0.176083   SS    
1376    2MASX J13085395+2730344            8.2    16.75   0.220974   E    
1377    SDSS J134719.23+114915.1           8.2    17.41   0.279850   Epec       
1378    2MASX J15093586+0757157            8.2    16.59   0.204342   E    
1379    2MASX J09373465+1036552            8.2    16.26   0.179424   SS    
1380    2MASX J09095608+5819209            8.2    15.70   0.142043   E    
1381    2MASX J08093749+2316385            8.2    17.39   0.273038   SS    
1382    2MASX J11100934+2357341            8.2    15.61   0.140612   E    
1383    2MASX J11053485+4105245            8.2    15.82   0.153334   E    
1384    LCRS B112440.2-024255              8.2    15.71   0.143289   E    
1385    2MASX J09341713+4200261            8.2    17.47   0.288473   E    
1386    2MASX J13382172+0929423            8.2    17.03   0.243039   SS    
1387    2MASX J11551407-0120412            8.2    17.39   0.277358   E    
1388    SDSS J123827.05+492105.3           8.2    16.56   0.205262   E    
1389    SDSS J110906.22+085621.3           8.2    17.35   0.273938   E    
1390    2MASX J12322911+5818000            8.2    17.49   0.291902   E    
1391    2MASX J11580685+5818097            8.2    17.13   0.253328   E    
1392    2MASX J12140193+3514012            8.2    16.89   0.233633   E    
1393    2MASX J11505046+2922414            8.2    17.37   0.276946   E    
1394    2MASX J13442322+1138566            8.2    14.70   0.095549   E    
1395    2MASX J13103930+2235023            8.1    16.87   0.231295   SS    
1396    2MASX J10410728+4315229            8.1    16.49   0.199531   E    
1397    2MASX J10194430-0038173            8.1    14.71   0.093688   E    
1398    2MASX J12283786+5008354            8.1    17.08   0.249799   E    
1399    2MASX J22302883+1341473            8.1    16.89   0.223492   E    
1400    2MASX J13275286+2009139            8.1    17.47   0.288000   E    
1401    2MASX J13240633+0533133            8.1    16.86   0.227100   E    
1402    2MASX J21331911-0638039            8.1    16.00   0.160546   E    
1403    2MASX J11233186+1542580            8.1    16.51   0.198486   E    
1404    2MASX J13510965+5843156            8.1    15.94   0.160576   E    
1405    2MASX J02485454+0111191            8.1    16.53   0.195785   E    
1407    2MASX J00294262-1011489            8.1    17.52   0.289587   E    
1408    SDSS J104800.48+151605.6           8.1    16.69   0.212755   E    
1409    SDSS J151721.02+603302.6           8.1    17.41   0.282475   SS    
1410    2MASX J14264257+5945405            8.1    16.91   0.234531   E    
1411    MCG +10-19-096                     8.1    13.97   0.071062   E    
1412    2MASX J21594449+0017289            8.1    17.39   0.271542   E    
1413    MCG +09-25-047                     8.1    17.02   0.244470   Epec     
1414    2MASX J13292948+3119453            8.1    16.99   0.242257   E    
1415    2MASX J08310113+0440195            8.1    16.17   0.173753   E    
1416    2MASX J10260165+5635457            8.1    16.49   0.200301   E    
1417    2MASX J09522530+3424025            8.1    17.27   0.268088   E    
1419    IC 3606                            8.1    15.19   0.115209   E    
1420    2MASX J13475962+3227100            8.1    16.79   0.223113   SS  
1421    2MASX J10032285+1123379            8.1    16.78   0.218455   E    
1422    4C +37.48                          8.1    15.96   0.161865   E    
1423    SDSS J215250.41+122159.2           8.1    17.52   0.273280   SS    
1424    2MASX J10193431+4100088            8.1    16.91   0.234783   E    
1426    2MASX J15104025+0048496            8.1    16.76   0.214240   E    
1427    SDSS J080224.68+253500.9           8.1    17.32   0.269598   E    
1428    2MASX J11162790+3813476            8.1    16.91   0.233491   SS    
1429    2MASX J14000349+0117160            8.1    17.07   0.243434   E    
1430    2MASX J11522532+4444140            8.1    17.55   0.296557   E    
1431    2MASX J10121210+5046503            8.1    15.57   0.138384   E    
1432    2MASX J15343991+0556176            8.1    17.08   0.241388   E    
1433    2MASX J15535909+4936359            8.1    16.85   0.228339   E    
1434    2MASX J13084556-0047178            8.1    16.37   0.188429   E    
1435    2MASX J23181976+0115033            8.1    16.81   0.217982   E    
1436    CGCG 215-022                       8.1    13.31   0.053270   E    
1437    2MASX J16141090+0857376            8.1    16.90   0.227946   E    
1438    2MASX J09242535+4234198            8.1    17.50   0.290931   E    
1439    2MASX J01065956+0015181            8.1    17.33   0.269833   E    
1440    SDSS J112946.88+234914.8           8.1    15.57   0.137798   E    
1441    2MASX J15520110+4317279            8.1    16.55   0.202813   E    
1442    2MASX J13135601-0034560            8.1    17.57   0.295714   E    
1443    2MASX J12531576+1817274            8.1    16.84   0.225361   E    
1444    2MASX J11442385+1557518            8.1    17.15   0.251733   E    
1445    2MASX J11273370+2101530            8.1    16.01   0.164416   E    
1446    2MASX J13504940+2943534            8.1    17.05   0.245818   E    
1447    2MASX J08482961+1058039            8.1    17.06   0.242854   E    
1448    2MASX J10344853+0424192            8.1    15.86   0.152495   E    
1449    SDSS J151436.24+055511.2           8.1    17.40   0.275000   E    
1450    SDSS J132743.82-031323.1           8.1    17.60   0.295193   SS    
1451    2MASX J12103402-0024451            8.1    16.28   0.181533   E    
1452    2MASX J23091768+1433511            8.1    17.66   0.253650   E    
1453    2MASX J14261304+1858464            8.1    16.69   0.211851   E    
1454    MCG +00-06-002                     8.1    14.27   0.079051   E    
1455    2MASX J15312701+1440507            8.1    17.01   0.237497   E    
1456    2MASX J13321164+1710543            8.1    16.61   0.207461   E    
1457    2MASX J09381666+1044508            8.1    17.01   0.239021   SS    
1458    2MASX J11344173+4629103            8.1    17.25   0.264275   E    
1459    2MASX J12575430-0158511            8.1    16.07   0.167757   E    
1460    2MASX J11295650+0832104            8.1    16.91   0.228859   E    
1461    2MASX J14503300+3510034            8.1    17.34   0.275505   E    
1462    2MASX J10323154+2211568            8.1    17.24   0.262170   E    
1463    2MASX J00451306+1528295            8.1    17.17   0.248746   E    
1464    2MASX J10041606+2958441            8.1    17.59   0.298435   SS    
1465    2MASX J12142586+0319295            8.1    17.06   0.246392   E    
1466    2MASX J08203267+0341412            8.1    17.10   0.249471   E    
1467    2MASX J16415609+4424023            8.1    17.54   0.296776   E    
1468    2MASX J16220041+1710399            8.1    17.07   0.242134   E    
1469    2MASX J11203472+0614363            8.1    17.41   0.270875   E    
1470    2MASX J17021393+6419540            8.1    16.81   0.222679   E    
1471    2MASX J16312132+4717324            8.1    16.92   0.233632   E    
1472    SDSS J222821.17+011410.4           8.1    17.64   0.293468   E    
1473    2MASX J15392995+3439152            8.1    16.91   0.231698   E    
1474    2MASX J16193468+0819252            8.1    15.89   0.150683   E    
1475    2MASX J08542755+5524598            8.1    17.09   0.246995   E    
1476    2MASX J08384387+0414510            8.1    16.69   0.210750   E    
1477    2MASX J10104735+4133460            8.1    16.99   0.240162   E    
1478    2MASX J14365542+6009444            8.1    17.06   0.247904   E    
1479    2MASX J13220810+3227009            8.1    17.24   0.263422   E    
1480    2MASX J14582285-0133388            8.1    16.97   0.228731   E    
1481    2MASX J15074934+3820464            8.1    16.56   0.203548   E    
1482    2MASX J01085879+1326010            8.1    15.74   0.145957   E    
1483    2MASX J10004491+1328284            8.1    16.65   0.208809   E    
1484    2MASX J16403286+2302461            8.1    17.37   0.267734   E    
1485    2MASX J11430322+5046219            8.1    17.40   0.279810   E    
1486    2MASX J12142070+4727133            8.1    17.11   0.252124   E    
1487    2MASX J02491189-0048481            8.1    17.40   0.272002   E    
1488    2MASX J09541020-0111404            8.1    15.65   0.138446   E    
1489    SDSS J144741.46+530115.7           8.1    17.45   0.286348   E    
1490    2MASX J08164043+3340182            8.1    17.06   0.238297   Epec   
1491    2MASX J10051339+2242214            8.1    17.08   0.243933   E    
1492    2MASX J07381980+4504281            8.1    15.91   0.151517   E    
1493    2MASX J12303911+4114242            8.1    17.37   0.274894   E    
1494    2MASX J13450120+1801346            8.1    14.73   0.097040   E    
1495    B3 1435+456                        8.1    17.08   0.248000   E    
1496    2MASX J15473665+3318573            8.1    15.15   0.114326   E    
1498    SDSS J105558.38+131341.6           8.1    17.58   0.296781   E       
1499    2MASX J14493985-0134142            8.1    17.34   0.265987   E    
1500    2MASX J10095635+2611324            8.1    17.03   0.240939   SS    
1501    2MASX J09334777+2114362            8.1    16.17   0.172206   SS    
1502    2MASX J12514491+4137586            8.1    17.06   0.247326   E    
1503    2MASX J09414969+3744200            8.0    17.52   0.293185   E    
1504    2MASX J09081338+5900258            8.0    16.25   0.175852   E    
1505    2MASX J15494389+4146114            8.0    16.78   0.221040   E    
1506    SDSS J114433.28+395600.5           8.0    17.53   0.293447   E    
1507    2MASX J11221430+1750193            8.0    16.07   0.167600   E    
1508    2MASX J10092522+0949495            8.0    16.76   0.214470   E    
1509    2MASX J09151273-0026405            8.0    17.23   0.259792   E    
1510    2MASX J14061499+4223365            8.0    16.67   0.213232   E    
1511    2MASX J14162902+3745157            8.0    15.98   0.163239   E    
1512    SDSS J122944.64+272306.3           8.0    17.37   0.275721   SS    
1513    SDSS J101443.28+000150.8           8.0    17.36   0.272057   E      
1514    SDSS J080317.08+325932.6           8.0    17.18   0.248662   SS      
1515    2MASX J12282411+4758423            8.0    17.55   0.296495   E    
1516    2MASX J12335297+1511403            8.0    17.49   0.283569   E    
1517    2MASX J11563120+5421412            8.0    16.87   0.229607   E    
1518    2MASX J13412118+4732316            8.0    16.35   0.186276   E    
1519    2MASX J12422320+0722529            8.0    16.91   0.231067   E    
1520    2MASX J12354859+3919078            8.0    16.96   0.237013   SS    
1521    2MASX J11064746+1233214            8.0    17.31   0.270326   E    
1522    SDSS J141147.04+002420.2           8.0    17.28   0.261959   E    
1523    2MASX J09572071+0952525            8.0    17.47   0.280418   E    
1524    2MASX J10243813+3348370            8.0    17.32   0.271174   E    
1525    2MASX J14313702+5227247            8.0    17.50   0.291996   E    
1526    2MASX J11414166+0223211            8.0    16.94   0.233637   SS    
1527    2MASX J10234078+5205489            8.0    17.36   0.276106   E    
1528    2MASX J15135886+3700290            8.0    16.61   0.206531   E    
1529    SDSS J111510.86+002339.5           8.0    17.63   0.297342   E    
1530    2MASX J12195983+4850043            8.0    17.27   0.266881   E    
1531    2MASX J11035172+0029211            8.0    17.12   0.247585   E    
1532    2MASX J14252801+6241556            8.0    16.57   0.204579   E    
1533    IC 3557 NED01                      8.0    14.27   0.078900   E    
1534    B2 0758+28                         8.0    17.36   0.267234   E      
1535    2MASX J11160517+3303477            8.0    16.62   0.206078   SS    
1536    2MASX J11575620+1601310            8.0    17.49   0.279313   E    
1537    2MASX J08263279+4957377            8.0    16.26   0.177089   E    
1538    2MASX J10220535+0909250            8.0    16.42   0.188869   E    
1539    2MASX J21490457-0810488            8.0    15.58   0.134043   E    
1540    2MASX J14534133+3159032            8.0    17.06   0.245280   E    
1541    2MASX J09062135+4705249            8.0    16.31   0.184679   E    
1542    2MASX J15335776+5425389            8.0    16.65   0.210463   E    
1543    2MASX J12240209+4726336            8.0    16.35   0.187519   E    
1544    2MASX J14472834+5908314            8.0    17.04   0.245534   SS    
1545    SDSS J075607.06+383401.0           8.0    16.80   0.215529   E    
1546    2MASX J13435549+2440484            8.0    15.56   0.137258   SS    
1547    2MASX J08141310+5409022            8.0    17.39   0.273075   E    
1548    2MASX J08351784+2914116            8.0    16.86   0.222537   E    
1549    2MASX J08464747+0446053            8.0    17.07   0.241509   SS    
1550    2MASX J09190470+1119010            8.0    16.28   0.180230   E    
1551    2MASX J14534792+0434190            8.0    17.07   0.241404   E    
1552    2MASX J10292828+3046410            8.0    16.25   0.179085   E    
1553    2MASX J13064347+4628125            8.0    16.88   0.230900   E    
1554    2MASX J13422833+1157345            8.0    17.43   0.279133   SS    
1555    2MASX J09590594+1501151            8.0    16.62   0.205539   E    
1556    2MASX J11435857+2748244            8.0    17.49   0.286646   E       
1557    2MASX J09533005+1202102            8.0    15.45   0.129066   E    
1558    2MASX J20582876-0717450 NED01      8.0    17.33   0.259743   E    
1559    CGCG 122-067                       8.0    14.56   0.089008   SS      
1560    2MASX J14450362+2422472            8.0    16.32   0.182000   E    
1561    2MASX J00395069+1458423            8.0    17.64   0.283933   E    
1562    SDSS J163202.04+464545.7           8.0    17.55   0.294898   SS    
1563    SDSS J125336.87+400657.1           8.0    17.39   0.279023   E    
1564    2MASX J13284058+4547063            8.0    16.35   0.186322   E    
1566    2MASX J02040615-0916084            8.0    16.73   0.215592   E    
1567    2MASX J08224329+4532370            8.0    17.05   0.238171   E    
1568    SDSS J081303.05+132618.4           8.0    16.40   0.188274   E    
1569    2MASX J15081452+1312518            8.0    15.96   0.157253   E    
1570    2MASX J08074394+4453046            8.0    16.80   0.218142   E      
1571    2MASX J17065870+3140229            8.0    16.78   0.217555   E      
1572    2MASX J15253039+3535408            8.0    15.88   0.155055   E    
1573    2MASX J11265682+1102560            8.0    17.05   0.239670   E    
1574    2MASX J11475440+2816081            8.0    17.46   0.282961   E    
1575    2MASX J11230095+4358198            8.0    17.20   0.259843   E    
1576    2MASX J11092483+3936020            8.0    17.24   0.262956   E    
1577    2MASX J11091308+3049371            8.0    17.32   0.268701   E    
1578    2MASX J15294628+4408044            8.0    15.77   0.147824   E    
1579    2MASX J12572537+4912434            8.0    17.05   0.245159   E    
1580    SDSS J115856.26+092352.3           8.0    17.55   0.293119   E    
1581    2MASX J13232036+0608548            8.0    17.59   0.294626   E    
1582    2MASX J02151559+0058241            8.0    16.56   0.199671   E    
1583    2MASX J11483989+0658066            8.0    17.58   0.297859   E    
1584    2MASX J10540451+2525107            8.0    16.59   0.203809   E    
1586    2MASX J16213487+1319097            8.0    16.67   0.202616   E    
1587    2MASX J11273376+5910383            8.0    15.79   0.149595   E    
1588    2MASX J14302155+1908217            8.0    16.90   0.227201   E    
1589    2MASX J07505181+3445397            8.0    17.53   0.285663   E    
1590    2MASX J14255741+1857441            8.0    16.70   0.211530   E    
1591    2MASX J12295233+1140391            8.0    14.41   0.082800   E    
1592    2MASX J15005246-0220312            8.0    17.49   0.271898   E    
1593    2MASX J22265220-0056071            8.0    17.18   0.248313   E    
1594    2MASX J11122325+3358136            8.0    16.56   0.201658   E    
1595    2MASX J12574610+4632254            8.0    16.80   0.222394   E    
1596    2MASX J15124010+2540523            8.0    16.44   0.186085   E    
1597    2MASX J16321903+1758407            8.0    17.14   0.244016   E    
1598    2MASX J11252376+3618248            8.0    17.49   0.285361   E    
1599    2MASX J21270528-0658349            8.0    16.98   0.221527   E      
1600    SDSS J115155.92+104634.7           8.0    17.47   0.283039   SS    
1601    2MASX J14583359+4729510            8.0    14.46   0.085479   E    
1602    2MASX J22433324+1308517            8.0    17.01   0.235545   E    
1603    2MASX J03563776-0638014            8.0    16.80   0.209398   E    
1604    2MASX J15095930+4958012            8.0    17.30   0.269463   E    
1605    2MASX J15410897+2343037            8.0    16.88   0.221484   E    
1606    SDSS J121644.34+122450.5           8.0    17.22   0.257144   SS     
1607    SDSS J130454.84+100011.6           8.0    17.19   0.255875   E    
1608    SDSS J040422.91-054134.9           8.0    17.27   0.250635   SS    
1609    2MASX J12071504+1713488            8.0    16.87   0.221788   E    
1610    2MASX J08302311+4744471            8.0    17.10   0.243735   E    
1611    2MASX J00380781-0109365            8.0    16.65   0.208695   SS    
1612    2MASX J12004632+4834375            8.0    17.38   0.274751   E    
1613    2MASX J11220880+2730177            8.0    17.22   0.260364   E    
1614    2MASX J10553814+1100202            8.0    15.45   0.130129   E    
1615    2MASX J12251987+0758564            8.0    17.13   0.250551   E    
1616    2MASX J14015072+2010090            8.0    16.67   0.208070   E    
1662    SDSS J085123.17-002148.7           7.9    17.59   0.295481   Epec       
#-------------------------------------------------------------------------------
#-------------------------------------------------------------------------------

